Next-to-minimal $R$-symmetric model: Dirac gaugino, Higgs mass and invisible width

We study a singlet extension of the minimal $U(1)_R$ symmetric model, which shares nice properties of Dirac gauginos and $R$-symmetric Higgs sector. At the same time, a superpotential coupling of $R$-charged singlet to the Higgs doublets can give a substantial contribution to the Higgs boson mass. We show that the 125 GeV Higgs boson is consistent with perturbative unification, even if the SUSY scale is as low as 1 TeV and if the $D$-term Higgs potential is suppressed as is often the case in Dirac gauginos. The model also contains a light scalar and fermion, pseudo-moduli and pseudo-Goldstino: The former gets a mass mainly from SUSY breaking soft terms, in addition to a small explicit $R$-symmetry breaking for the latter. We examine how the Higgs mass and width are affected by these light degrees of freedom. Specifically we find thatdepending on parameters of $R$-charged Higgses, the pseudo-moduli lighter than a half of the SM-Higgs boson mass is still allowed by the constraints from invisible decays of the $Z$ and Higgs bosons. We also find that such a light scalar can reduce the Higgs boson mass, at most by a few percents.

==> v2_changelog/diff_main20160210a-322a <==
37c37,39
< Niigata University,~Niigata, 950-2181, Japan}
---
> Niigata University,~Niigata, 950-2181, Japan\\[20pt]
> \medskip
> }
87,91c89,93
< \input sec1_intro20160107a.tex
< \input sec2_setup20160107a.tex
< \input sec3_triviality20160107a.tex
< \input sec4_width20160107b.tex
< \input sec5_conclusion20160107a.tex
---
> \input sec1_intro20160107b.tex
> \input sec2_setup20160107b.tex
> \input sec3_triviality20160107b.tex
> \input sec4_width20160107c.tex
> \input sec5_conclusion20160107b.tex
122,124c124,126
< \input appendix1_20160104a_RGE.tex
< \input appendix2_20160104a_gaugino.tex
< \input appendix3_20160104a_unification
---
> \input appendix1_20160104b_RGE.tex
> \input appendix2_20160104b_gaugino.tex
> \input appendix3_20160104b_unification
126c128
< \input sec6_reference20160107a.tex  
---
> \input sec6_reference20160107b.tex  


==> v2_changelog/diff_sec1_intro20160107a-b <==
28c28
< models with Dirac gaugino has recently attracted much attention
---
> models with Dirac gaugino have recently attracted much attention
71c71
< in Ref.~\cite{Bertuzzo:2014bwa,Diessner:2014ksa} showing that
---
> in Refs.~\cite{Bertuzzo:2014bwa,Diessner:2014ksa} showing that
93c93
< the next--to--minimal $R$-symmetric model in short;
---
> the next--to--minimal $R$-symmetric model for short;
126c126
< we assume that explicit $R$ symmetry breaking
---
> we assume tha explicit $R$ symmetry breaking
132c132
< of order of a few GeV, for instance.
---
> of the order of a few GeV, for instance.
145c145
< were studied to some details;
---
> were studied in some details;
178c178
< but such enhancement is limited by triviality bound
---
> but such enhancement is limited by the triviality bound
180c180
< These are some important differences, however.
---
> There are some important differences, however.
247c247
< The constraint from the $Z$ decay to pseudo-Goldstino pair
---
> The constraint from the $Z$ decay to a pseudo-Goldstino pair
250c250
< We also examine the invisible Higgs decay to pseudo-moduli pair,
---
> We also examine the invisible Higgs decay to a pseudo-moduli pair,


==> v2_changelog/diff_sec2_setup20160107a-b <==
46c46
< which we assume to be of order of the weak scale.
---
> which we assume to be of the order of the weak scale.
50c50
< A dimension two parameter $f$ of order of the weak scale 
---
> A dimension--two parameter $f$ of the order of the weak scale 
62c62
< We will refer to it as \textit{singlet Yukawa coupling}.
---
> We will refer to this as \textit{singlet Yukawa coupling}.
66c66
< to discuss implications of this singlet Yukawa coupling
---
> to discuss the implications of this singlet Yukawa coupling
98,99c98,99
< We also put a sign factor $\eta_u=+1$ and $\eta_d=-1$
< so that the neutral components has plus sign.
---
> We also put sign factors $\eta_u=+1$ and $\eta_d=-1$
> so that the neutral components have plus signs.
116c116
< to reproduce the lightest Higgs mass of $125\nunits{GeV}$.
---
> in reproducing the lightest Higgs mass of $125\nunits{GeV}$.
331c331
< at the cost of loosing the supersoftness 
---
> at the cost of losing the supersoftness 
363,364c363,364
< Here $V_F$ and $V_A$  corresponds, respectively,
< to the superpotential \eq{eq:W:Higgs} %\eq{eq:higgs:secter:superpot}
---
> Here $V_F$ and $V_A$  correspond, respectively,
> to the superpotentials \eq{eq:W:Higgs} %\eq{eq:higgs:secter:superpot}
376c376
< which reads,
---
> which read,
568c568
< can give a tiny gaugino components \cite{Morita:2012kh}.
---
> can give a tiny gaugino component \cite{Morita:2012kh}.
647c647
< so that $m^2_\phi$ shows some interesting behaviour.
---
> so that $m^2_\phi$ shows some interesting behavior.


==> v2_changelog/diff_sec3_triviality20160107a-b <==
207c207
< Being so,
---
> This being so,
530c530
< and also in the MRSSM \cite{Diessner:2015yna}.
---
> and also in the minimal $R$-symmetric model (MRSSM) \cite{Diessner:2015yna}.
600c600
< the contour of the Higgs mass $125\nunits{GeV}$
---
> the contours of the Higgs mass $125\nunits{GeV}$
616,617c616
< the minimal $R$-symmetric model (MRSSM),
< where 
---
> the MRSSM, where 
726c725
< where $m_{R_{u,d}}$ are the soft mass of $R_{u,d}$.
---
> where $m_{R_{u,d}}$ are the soft masses of $R_{u,d}$.
831c830
< The matching to the SM with a light moduli is assumed
---
> the matching to the SM with a light moduli is assumed


==> v2_changelog/diff_sec4_width20160107b-c <==
10c10
< we examine how the present model are constrained from 
---
> we examine how the present model is constrained from 
95c95
< These behaviour can be understood from our estimate 
---
> These behavior can be understood from our estimate 
118,119c118,119
< $\mu=400{\rm GeV}$ in the left,
< while $m_R=300{\rm GeV}$ in the right.
---
> $\mu=400\nunits{GeV}$ on the left,
> while $m_R=300\nunits{GeV}$ on the right.
268c268
< The quartic coupling $g_{hh\phi\phi}$ cam be found
---
> The quartic coupling $g_{hh\phi\phi}$ can be found
270c270
< we omit it here since it is irrelevant for later purpose.
---
> we omit it here since it is irrelevant for later purposes.
501c501
< as a functions of $\mu$ and soft mass $m_R$ of $R_{u,d}$.
---
> as a function of $\mu$ and soft mass $m_R$ of $R_{u,d}$.
526c526
< %%as a functions of the common soft mass $m_R$.
---
> %%as a function of the common soft mass $m_R$.
714c714
< a pair of the pseudo-moduli $\phi$
---
> a pair of pseudo-moduli $\phi$
824,825c824,825
< The reason for this behaviour is that
< the lighter $\phi$ implies the smaller $g_{h\phi\phi}$ coupling.
---
> The reason for this behavior is that
> lighter $\phi$ implies smaller $g_{h\phi\phi}$ coupling.
857c857
< The purple and Gray regions are excluded 
---
> The purple and gray regions are excluded 
905c905
< and implies $0.2\,\%$ enhancement ($0.8\,\%$ reduction)
---
> and implies $0.2\%$ enhancement ($0.8\%$ reduction)
909c909
< leads to the $D$-term suppression $\suppress{D}=1/2$.
---
> lead to the $D$-term suppression $\suppress{D}=1/2$.


==> v2_changelog/diff_sec5_conclusion20160107a-b <==
45c45
< in a small $\tan\beta$ region
---
> in the small $\tan\beta$ region
51c51
< gives substantial improvement of the Higgs mass
---
> give substantial improvement to the Higgs mass
57c57
< and that there are broader parameter region
---
> and that there is broader parameter region
77c77
< again even without $D$-term.
---
> again even without the $D$-term.
92c92
< that the Higgs invisible width is within the current bound
---
> in which the Higgs invisible width is within the current bound
96c96
< than $\lambda v$ of order of $100\nunits{GeV}$.
---
> than $\lambda v$ of the order of $100\nunits{GeV}$.
100,101c100,101
< including full SUSY spectrum 
< and higher loop corrections are desired.
---
> including the full SUSY spectrum 
> and higher-loop corrections are desired.
115,117c115,117
< Detailed studies about the adjoint Yukawa couplings
< and their upper bound should be done.
< On a theoretical side,
---
> Detailed studies on the adjoint Yukawa couplings
> and their upper bounds should be done.
> On the theoretical side,
122c122
< cosmology of the singlet extended $R$-symmetric model
---
> the cosmology of the singlet extended $R$-symmetric model


==> v2_changelog/diff_sec6_reference20160107a-b <==
416,418c416,418
<   ``New Phenomena in Lepton-Hadron Physics'', 
<   D.E.C.~Fries and J.~Wess eds., Plenum, New York, U.S.A. (1979),
<   pg.~303.
---
>   ``\textit{New Phenomena in Lepton--Hadron Physics}'', 
>   eds. D.E.C.~Fries and J.~Wess (Plenum, New York, 1979),
>   p.~303.
421,423c421,423
<   ``Fifth Workshop on Grand Unification'', 
<   K.~Kang, H.~Fried and P.~Frampton eds., 
<   World Scientific, Singapore (1984), pg.~88.
---
>   ``\textit{Fifth Workshop on Grand Unification}'', 
>   eds. K.~Kang, H.~Fried and P.~Frampton 
>   (World Scientific, Singapore, 1984), p.~88.
436,437c436,437
<   ``The Study of ~q(L) ~q(L) production at CERN LHC 
<   in the l+- l+- channel and sensitivity to other models,''
---
> %  ``The Study of ~q(L) ~q(L) production at CERN LHC 
> %  in the l+- l+- channel and sensitivity to other models,''


==> v2_changelog/sec1_intro20160107a.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
\label{sec:introduction}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Low--energy supersymmetry (SUSY) is a fascinating idea
since it was proposed as a solution to the hierarchy problem
and further supported by a sign of gauge coupling unification.
Such idea is now challenged, however,
since no signal for SUSY particles has been 
%found 
reported yet
at the Large Hadron Collider (LHC).
The discovery of the Standard Model (SM)-like Higgs boson
at $125\nunits{GeV}$ also indicates that
SUSY would be heavy \cite{Giudice:2011cg}, if exists,
since the identification of the discovered boson
with the lightest Higgs boson in the Minimal SUSY SM (MSSM) 
requires large radiative corrections from the top squarks.


An $R$-symmetric realization of low-energy SUSY 
provides an alternative to the MSSM \cite{Hall:1990hq,Randall:1992cq}.
In particular,
models with Dirac gaugino has recently attracted much attention
%and is actually attractive 
in several respects:
``supersoftness'' of scalar masses \cite{Fox:2002bu}, 
``supersafeness'' of squark production 
\cite{Heikinheimo:2011fk,Kribs:2012gx},
as well as 
improved properties in flavor sector \cite{Kribs:2007ac}:
The adjoint chiral multiplets,
including Dirac partners of the MSSM gauginos,
also contain adjoint scalars, 
$\mathcal{N}=2$ partners of the gauginos,
which have a suitable coupling to cancel UV divergences
of scalar masses.
This can improve naturalness property of the Higgs potential.


In the minimal setup of $U(1)_R$-symmetric model \cite{Kribs:2007ac},
we introduce an $R$-partner to each gaugino and Higgsino.
An $R$-partner of the MSSM gaugino $\lambda_{a=3,2,1}$,
is contained in an adjoint chiral multiplet,
$\mathcal{A}_3=O$, $\mathcal{A}_2=T$ and $\mathcal{A}_1=S$,
while an $R$-partner of the MSSM Higgs doublet, $H_{i=u,d}$,
is denoted by $R_{i=u,d}$.
The minimal $R$-symmetric model is known to have advantages
of suppressing flavor and CP violations 
\cite{Hisano:2006mv,Kribs:2007ac,Fok:2010vk,Dudas:2013gga};
Phenomenological study \cite{Choi:2010an}
and electroweak (EW) baryogenesis \cite{Kumar:2011np,Fok:2012fb}
was also discussed.
% in the minimal $R$-symmetric Higgs sector.
%See Refs.~\cite{Frugiuele:2012pe,Morita:2012kh}
See Refs.~\cite{Frugiuele:2012pe,Morita:2012kh,Chakraborty:2013gea} 
for $R$-symmetric models with different $R$-charge assignments,
and Ref.~\cite{Benakli:2014cia}
for a minimal SUSY model of Dirac gaugino
with and without $R$-symmetry.


%In addition,
%%it was pointed out 
%it was claimed in Ref.~\cite{Bertuzzo:2014bwa,Diessner:2014ksa} that
An important step was made 
in Ref.~\cite{Bertuzzo:2014bwa,Diessner:2014ksa} showing that
the $125\nunits{GeV}$ Higgs mass can be accommodated
if the $SU(2)\times U(1)$ adjoints $\mathcal{A}_{1,2}$ have
sufficiently large couplings to the Higgs pairs $R_iH_i$:
Such adjoint Yukawa couplings can also relax 
the suppression of $SU(2)\times U(1)$ $D$-term potential,
which is known as a drawback of supersoft SUSY breaking models.
Notice, however, that
although marginally allowed \cite{Diessner:2015yna},
such large adjoint couplings are generally in tension with 
EW precision measurements,
as in the muless SUSY SM \cite{Nelson:2002ca}.
%but detailed analysis shows that they are marginally allowed.
Perturbativity constraints should also be taken into account.
%(as was done for a non $R$-symmetric model 
%with light chiral adjoints \cite{Kakizaki:2013eba}).


In the present paper,
we consider a singlet extension of 
the minimal $R$-symmetric SUSY SM, 
which may be called 
the next--to--minimal $R$-symmetric model in short;
It is actually a combination of Dirac gaugino
and an $R$-symmetric Higgs sector
proposed in Ref.~\cite{Izawa:2011hi}.
Unlike the conventional singlet extensions of the MSSM,
%whose motivation is to solve the $\mu$ problem,
the present model is not intended to explain
the origin of Higgsino mass terms.
Instead, we would like to examine 
how the lightest Higgs mass of $125\nunits{GeV}$
can be reproduced in our $R$-symmetric setup.
%by a singlet Yukawa coupling to the MSSM Higgs pair,
%consistently with perturbative unification.
Actually we show that
$125\nunits{GeV}$ Higgs mass 
can well be accommodated
by a singlet Yukawa coupling to the MSSM Higgs pair,
consistently with perturbative unification.
%within the triviality bound
%of the singlet Yukawa coupling.
We also examine to what extent
the adjoint Yukawa couplings can affect the results.
As is expected,
our solution requires small $\tan\beta$
so that the singlet coupling can give a substantial contribution
to the lightest Higgs mass;
it also favors small values for the adjoint Yukawa couplings.
Therefore our setup provides 
%a complimentary solution compared to 
an alternative to the known solution in the minimal $R$-symmetric model.


In the present work, 
we assume that explicit $R$ symmetry breaking
is very small, as was discussed in Ref.~\cite{Morita:2012kh};
Through coupling to supergravity,
the theory contains a small explicit breaking of $R$-symmetry,
characterized by the gravitino mass,
%of order of at most a few GeV.
of order of a few GeV, for instance.
Throughout the present paper,
we will neglect such explicit $R$-breaking effects,
including anomaly-mediated contribution to Majorana gaugino masses.
Cosmological issues will be discussed elsewhere.


The most characteristic feature of the present model 
is the presence of light degrees of freedom,
pseudo-moduli $\phi$ and pseudo-Goldstino $\psi$.
%In Ref.~\cite{Bertolini:2011tw,Morita:2012kh},
In Ref.~\cite{Bertolini:2011tw},
properties of such light degrees of freedom
were studied to some details;
A generic prediction there is that
the light scalar $\phi$ couples to the Higgs boson so strongly that
the Higgs decays almost invisibly to its pair.
%the Higgs invisible decay width is large.
We revisit this issue here,
and show that
there is a region of parameter space in which
a light scalar mode still exists
and, unlike the previous expectation,
the Higgs invisible width is within the present bound.
We explain why and when the coupling of the light scalars
to the Higgs boson becomes weak
thanks to its pseudo-moduli nature.


%\paragraph{Comparison with N(n)MSSM}

%We compare the present model with the NMSSM~%
%[Note: no kappa, no A term, ...]


It is worth mentioning that
the present model has a similarity
with the conventional singlet extensions of the MSSM
--- the NMSSM
\cite{Ellwanger:2009dp,Badziak:2013bda,Ellwanger:2012ke,%
Kobayashi:2012ee,Goodsell:2014pla},
the nMSSM \cite{%
Panagiotakopoulos:1999ah,Panagiotakopoulos:2000wp,Ishikawa:2014owa}
or the PQ-NMSSM \cite{Jeong:2011jk,Jeong:2012ma,Choi:2013lda}:
the SM-like Higgs boson mass can be enhanced
at small $\tan\beta$,
but such enhancement is limited by triviality bound
of the singlet coupling(s).
These are some important differences, however.
First of all,
in the present setup,
%the singlet has nonzero $R$-charge so that
%it can not mix with the SM-like Higgs boson
%modulo small explicit $R$-symmetry breaking effects.
the SM-like Higgs boson should be the lightest mass eigenstate
in the $R$-neutral scalars,
since the approximate $R$-symmetry forbids the mixing
to the $R$-charged scalars.
The $R$-symmetry also forbids $A$-terms 
that could be used for enhancing the Higgs mass.
Moreover,
in the conventional models,
the Higgsino mass term is forbidden 
by imposing some symmetries
while our model contains $R$-invariant Higgsino mass parameters
from the start.
These mass terms, on a theoretical side,
trigger spontaneous SUSY breaking in the Higgs sector
\cite{Izawa:2011hi};
%which deserves further study by itself.
At the same time, the mass terms 
can suppress (unwanted) mixings between
the singlet and doublet states in the $R$-charged sector.
We thus expect that
the resulting phenomenology can be quite different.


%\paragraph{Organization}


The present paper is organized as follows.
%
In \S\ref{sec:setup},
we introduce out setup for a singlet extension of the minimal
$R$-symmetric SUSY SM and describe its characteristic features,
the existence of light degrees of freedom 
related to a pseudo-moduli direction.
We also give a brief review of aspects of Dirac gaugino
in supersoft SUSY breaking,
including the suppression of $D$-term quartic scalar potential.
%In Sec.~\ref{sec:Higgs:mass} 
In \S~\ref{sec:triviality} 
we discuss how the $125\nunits{GeV}$ Higgs boson can be compatible
with perturbative unification.
We use two-loop renormalization group equations (RGE's)
but mainly consider the case
in which the SUSY particle masses
can be treated 
%by a single representative mass scale $\MS$.
by a single mass threshold $\MS$.
We calculate the lightest Higgs mass
in the RG approach:
At the scale $\MS$, we match the $R$-symmetric model
%to the low-energy effective theory
to the minimal SM
by taking the decoupling limit of the heavier Higgs states.
We also take into account various effects
including adjoint Yukawa interactions and 
a possibility of a light pseudo-moduli below the matching scale.


The constraints from 
invisible decay of the $Z$ and SM-like Higgs bosons
are examined in \S~\ref{sec:decay}.
%We find that 
The constraint from the $Z$ decay to pseudo-Goldstino pair
can be satisfied if 
the $R$-symmetric Higgsino mass parameters are not too small.
We also examine the invisible Higgs decay to pseudo-moduli pair,
and find that
there is a region of parameter space
corresponding to a pseudo-moduli that 
is lighter than a half of the SM-like Higgs boson mass,
and such a light pseudo-moduli has very suppressed coupling
to the Higgs boson(s).
The final section is devoted to conclusion and discussion.
Necessary tools for the RG analysis
and some detailed discussion about 
gauge coupling unification and 
Dirac gaugino mass threshold
%the matching condition to low-energy effective theory
%including the light pseudo-moduli
are given in Appendices.



==> v2_changelog/sec2_setup20160107a.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Dirac Gaugino and 
Next-to-minimal $R$-symmetric Higgs Sector}
\label{sec:setup}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


We consider the theory invariant under $U(1)_R$
under which all the SM fields are neutral.
The $R$-symmetric superpotential proposed in Ref.~\cite{Izawa:2011hi}
%and further studied in Refs.~\cite{Bertolini:2011tw,Morita:2012kh}
is given by $W = W_H + W_Y$, where\,\footnote{%
The $R$-charged fields $R_0$, $R_u$ and $R_d$
were denoted in Ref.~\cite{Izawa:2011hi}
by $X_0$, $X_1$ and $X_2$, respectively.
Accordingly the Higgsino mass parameters
$\mu_u$ and $\mu_d$ here correspond to $\mu_1$ and $-\mu_2$ there;
%Note that 
we have flipped the sign of $\mu_d$ term
so that
all the neutral components have the same sign.
Note also that the parameters, $\lambda$, $\mu_{u,d}$, $f$, 
can be made real and positive
by field redefinition of $R_{0,u,d}$ and $H_{u,d}$.
} 
\begin{align} 
% W &= W_H + W_Y
% \ ,
% \label{eq:superpot}\\
  W_H
  &= R_0\left(f+\lambda H_uH_d\right)
   + \mu _uR_uH_u-\mu_dR_dH_d
   \ ,
 \label{eq:W:Higgs} % \label{eq:higgs:secter:superpot}
\\
 W_Y
 &= y^{ij}_u Q_iU^c_jH_u + y^{ij}_d Q_iD^c_jH_d + y^{ij}_e E^c_iL_jH_d
 \ .
 \label{eq:W:Yukawa} % \label{eq:Ykawa:superpot}
\end{align}
Here $H_{u,d}$ are the MSSM Higgs doublets,
$R_{u,d}$ are their $R$-partners of $R$ charge $+2$, and
$\mu_{u,d}$ are $R$-invariant Higgsino mass parameters
which we assume to be of order of the weak scale.
%the linear term in \Eq{eq:higgs:secter:superpot}
%the linear term in \Eq{eq:W:Higgs}
%triggers the electroweak symmetry breaking (EWSB)...
A dimension two parameter $f$ of order of the weak scale 
can act as additional source of (super)symmetry breaking,
as was further studied in Refs.~\cite{Bertolini:2011tw,Morita:2012kh}.
A possible origin of these mass parameters
was also discussed in Ref.~\cite{Izawa:2011hi}.
%Moreover, the superpotential~\ref{eq:higgs:secter:superpot} 
%Moreover, the superpotential~\ref{eq:W:Higgs} 
%induces visible SUSY breaking~\cite{Izawa:2011hi}.
%Finally, 
In addition, we introduce a gauge singlet $R_0$ of $R$-charge 2,
which has an nMSSM-like coupling $\lambda$
to the MSSM Higgs doublets $H_{u,d}$.
We will refer to it as \textit{singlet Yukawa coupling}.
%(or nMSSM-like coupling).
%(although it looks like a similar coupling in the NMSSM or nMSSM).
It is the purpose of the present paper
to discuss implications of this singlet Yukawa coupling
in the Higgs mass and decay width.
%Note that the parameters, $\lambda$, $\mu_{u,d}$, $f$, 
%can be made real and positive
%by field redefinition of $R_{0,u,d}$ and $H_{u,d}$.


The $U(1)_R$ symmetry forbids the usual Majorana mass terms
for the MSSM gauginos.
To allow Dirac gaugino mass terms
we introduce chiral supermultiplets $\mathcal{A}_a$
belonging to the adjoint representation of
the SM gauge group $SU(3)_c \times SU(2)_L \times U(1)_Y$,
where $a=3,2,1$ is a gauge index;
Explicitly,
$\mathcal{A}_3=O$ is an $SU(3)$-octet, 
$\mathcal{A}_2=T$ an $SU(2)$-triplet, $\mathcal{A}_1=S$ a singlet.
%$\mathcal{A}_1=S$, $\mathcal{A}_2=T$, $\mathcal{A}_3=O$.
%which we denote collectively by $\mathcal{A}_a$.
We denote their fermion and scalar components
by $\chi_a$ and $A_a=\left(\sigma_a+i\pi_a\right)/\sqrt{2}$, respectively.
Matter contents and $R$-charge assignment are 
summarized in the Table.~\ref{tab:contents}.


\input table1_content20160104a.tex


In the presence of these adjoint chiral multiplets,
we can add the following superpotential\,\footnote{
Following the existing literature, we put a normalization factor
$k_{2}=2$ for $SU(2)$-adjoint Yukawa terms while $k_{1}=1$ for $U(1)$.
We also put a sign factor $\eta_u=+1$ and $\eta_d=-1$
so that the neutral components has plus sign.
}
\begin{align} 
% W_{\mathrm{ad}}
 W_A
 &=\sum_{a=2,1}\sum_{i=u,d}
   \eta_i k_a\lambda ^i_a R_i\mathcal{A}_a H_i
\nonumber\\
 &= 2\lambda ^u_T R_u T H_u - 2\lambda ^d_T R_d T H_d 
   + \lambda ^u_S R_u S H_u - \lambda ^d_S R_d S H_d 
   \ ,
\label{eq:W:adjoint} % \label{eq:adjoint:Yukawa:superpot}
\end{align}
which we refer to as \textit{adjoint Yukawa terms}
(although $\mathcal{A}_1=S$ is actually a singlet).
In Refs.~\cite{Bertuzzo:2014bwa,Diessner:2014ksa},
these terms play a central role
to reproduce the lightest Higgs mass of $125\nunits{GeV}$.
In the present model, however,
it is not these adjoint Yukawa terms but 
the singlet Yukawa term 
in \Eq{eq:W:Higgs} %\Eq{eq:higgs:secter:superpot}
that is important for the Higgs mass.


%The superpotential $W=W_H+W_Y+W_{\mathrm{ad}}$
The superpotential $W=W_H+W_Y+W_A$
is not completely general one
%that is allowed by the symmetries of the model.
that is allowed by the $R$-symmetry.
%The basic assumption here is that
Our assumption here is that
there is no superpotential term
that is quadratic in adjoint chiral multiplets $\mathcal{A}_a$,
such as $R_0S^2$ and $R_0T^2$.
We also assume that
the mixing mass term of $S$ and $R_0$ 
does not arise after GUT symmetry breaking.
%To justify these assumptions,
%it would be necessary to discuss a possible embedding of the model
To justify these assumptions would require 
a concrete embedding of the model into grand unified theories (GUT's):
%but it is beyond the scope of the present work.
%which we do not attempt here.
%[A possible justification of these assumption will be discussed elsewhere.]
Here we just note that an interesting possibility is provided
by an orbifold-type model \cite{Kojima:2011ad},
which does contain light chiral adjoints after GUT symmetry breaking.




%%We introduce the R-charged Higgses 
%%because usual higgsino mass term (mu term) is forbidden by R-symmetry. 
%%%\footnote{If you want to know $\mu$-term less SUSY model, 
%%%you should reference of \cite{Nelson:2002ca}}
%%We also introduce $R_0$ 
%%in order realize the lightest Higgs mass of 125 GeV
%%through additional Higgs 4 point interaction term.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Supersoft SUSY Breaking and Suppression of $D$-term} 
\label{subsec:supersoft}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Dirac gaugino mass terms are generated through
so-called supersoft operator~\cite{Polchinski:1982an,Fox:2002bu}
\begin{align}
 \mathcal{L}_{\mathrm{SS}}
 = \sum_{a=3,2,1}\int d^2\theta 
   \frac{\sqrt{2}\,g_a}{\Lambda _D}\,
   \mathcal{W}^\alpha_X \mathcal{W}^a_\alpha \mathcal{A}_a
 + \mathrm{H.c.} \ ,
 \label{eq:DG:superpot}
\end{align}
where 
%$\mathcal{A}_a$ are chiral adjoint fields of  
%$U(1)_Y$, $SU(2)_L$ and $SU(3)_c$ and 
$\mathcal{W}_X$ is the gauge field strength of a hidden sector $U(1)_X$ 
whose nonvanishing $D$-term\,\footnote{
See Refs.~\cite{Itoyama:2011zi,Itoyama:2012fk}
for a mechanism of $D$-term dynamical SUSY,
and Refs.~\cite{Alves:2015kia,Alves:2015bba}
for a mechanism for generating the supersoft operator
through a Wess--Zumino--Witten term.
Note that a constant shift in adjoint scalars
is not allowed by the supersoft operator \eq{eq:DG:superpot}.
%as well as adjoint scalar mass terms.
} 
is a source of SUSY breaking
and $\Lambda_D$ is a cutoff scale 
at which the above operator is generated.
A vacuum expectation value (VEV) of $U(1)_X$ $D$-term, 
$\VEV{D_X}$, gives
\begin{align} 
 \mathcal{L}_{\mathrm{SS}}
 \longrightarrow{} 
 - \Bigl\{
	 m_{D_a}\lambda_a \chi_a + \mathrm{H.c.}
   \Bigr\}
	 - 2m_{D_a} D_a \sigma_a 
  \ ,
 \label{eq:DG:lag}	 
\end{align}
where $m_{D_a}=g_a\VEV{D_X}/\Lambda_D$ is a Dirac mass of 
gaugino $\lambda_a$ and adjoint fermion $\chi_a$
(at the scale $\Lambda_D$);
At the same time, the second term gives rise to 
the mass term of the real part $\sigma_a$ of the adjoint scalar and 
the trilinear scalar interactions of $\sigma_a$ to other scalars.
The latter has important consequences,
supersoftness and $D$-term cancellation,
which we review shortly.


If the $U(1)_X$ $D$-term is the only source of SUSY breaking,
a soft scalar mass in the visible sector is UV finite.
Such supersoft contribution is given by \cite{Fox:2002bu}
\begin{align}
\delta m^2\fun{\varphi_i}
 &= \sum_{a=3,2,1}
    \frac{4C_2^a\fun{\varphi_i}g^2_a}{16\pi^2}\,m_{D_a}^2
%    \log\frac{4m_{D_a}^2+\delta m_{\sigma_a}^2}{m_{D_a}^2}
    \log\frac{m_{\sigma_a}^2}{m_{D_a}^2}
    \ ,
\label{eq:supersoft:scalarmass}
\end{align}
where $C_2$ is a quadratic Casimir for a scalar $\varphi_i$ and 
%$\delta m^2_{\sigma_a}$ is additional mass of 
$m^2_{\sigma_a}$ is the mass squared of 
the adjoint scalar $\sigma_a$.
Note that its pseudo-scalar partner $\pi_a$ 
%remains massless at this level.
does not receive a mass from the supersoft operator \eq{eq:DG:superpot}.
Although the $U(1)_R$ symmetry forbids 
supersymmetric mass term of $\mathcal{A}_a$,
its scalar components 
$A_a=\left(\sigma_a+i\pi_a\right)/\sqrt{2}$ can get a mass 
from holomorphic and non-holomorphic soft mass terms
\cite{Carpenter:2010as,Csaki:2013fla,Alves:2015kia,Alves:2015bba}.
In addition,
$SU(3)\times SU(2)$ adjoints receive 
finite loop corrections \eq{eq:supersoft:scalarmass} to their masses.
We denote the resultant masses of adjoint scalars
by $m_\sigma^2=4m_D^2+\delta m_\sigma^2$ and $m_\pi^2$, respectively.
We will assume that
these adjoint scalars have large enough masses 
to prevent them from developing a nonzero VEV
%%\rlap,\footnote{
%%[memo]:
%%It the $U(1)_Y$-adjoint scalar develops a non-zero VEV $\VEV{S}$,
%%the $\mu_{u,d}$ terms are generated, 
%%$\mu_{u,d}=\lambda_S^{u,d}\VEV{S}$,
%%but a worry is that
%%the singlet VEV would induce a large
%%kinetic mixing $\mathcal{W}_X^\alpha\mathcal{W}_{Y\alpha}$.
%%}
especially in the presence of the adjoint Yukawa terms
\eq{eq:W:adjoint}. %\eq{eq:adjoint:Yukawa:superpot}.
%[We also note that
%a large $\lambda_{ai}$ is not favored
%in view of the lightest Higgs mass of $125\nunits{GeV}$,
%as we see in Sec.~\ref{sec:triviality}.]


%Another characteristic feature of models of Dirac gaugino
Another characteristic feature of Dirac gaugino models
is the suppression of the $D$-term scalar potential \cite{Fox:2002bu}.
Here let us recall it in the absence of adjoint Yukawa terms.
Then the relevant terms are
\begin{align} 
 V_D
  =  \sum_{a} \frac{1}{2}
     \left[ 
       2m_{D_a} \sigma _a - \sum_i \varphi^*_i g_a T^a \varphi_i
     \right]^2
   + \sum_a\!\left[
        \frac{1}{2}\,\delta m_{\sigma_a}^2 \left(\sigma_a\right)^2
      + \frac{1}{2}\,m_{\pi_a}^2   \left(\pi_a\right)^2
     \right]
     \ ,
\end{align}
%where $\sigma_a$ are normalized real part of adjoint scalar.  
where $\varphi_i$ is a generic scalar field.
%and the summation over $a=3,2,1$ is implied.
If the adjoint scalar $\sigma_a$ can be regarded as heavy enough
to be integrated out,
the effective $D$-term potential is given by
\begin{align} 
 V_D^{\mathrm{eff}}
\ =\ \sum_{a}\suppressionD{D_a}
     \frac{g_a^2}{2}
     \left[\sum_i \varphi^*_i T^a \varphi_i\right]^2
     \ , \qquad
\suppressionD{D_a}
\ \equiv\ \frac{\delta m^2_{\sigma_a}}{4m^2_{D_a}+\delta m^2_{\sigma_a}}
     \ ,
 \label{eq:Dterm:pot}
\end{align}
where $\suppressionD{D_a}$ is a suppression factor
%%\,\footnote{
%%In principle, $\delta m_{\sigma_a}^2$ can be negative,
%%but in such a case, 
%%it would be more appropriate to treat $\sigma_a$ as a light degrees of
%%freedom.
%%} 
between $0$ and $1$.
%%For instance,
%%$\varepsilon_{D_1}=0$ and $\varepsilon_{D_2}\approx 7.3\times 10^{-3}$
%%in the supersoft limit in which
%%%$\delta m^2_{\sigma_2}$ is given solely by the finite loop correction
%%%\eq{eq:supersoft:scalarmass}
%%\begin{align}
%%\delta m^2_{\sigma_2}
%%\ =\ \frac{4\alpha_2}{2\pi}\,m_{D_2}^2 \log{4}
%%\ \approx\ \left(0.17 m_{D_2}\right)^2
%%    \ . 
%%\end{align}
Such suppression of the quartic $D$-terms 
is not welcome in low-scale supersymmetry\,\footnote{
%See however Ref.~\cite{Fox:2014moa} for an interesting application.
See however Refs.~\cite{Unwin:2012fj,Fox:2014moa} for an interesting application.
}
%since it implies 
%the Higgs quartic coupling is suppressed
%and it is more difficult to reproduce $125\nunits{GeV}$ Higgs mass.
and can be avoided by assuming
large additional contribution $\delta m^2_{\sigma_a}$
to the adjoint scalar masses.
[Of course, this can be done 
at the cost of loosing the supersoftness 
\cite{Arvanitaki:2013yja,Csaki:2013fla}.]
%%$\suppressionD{a}\to 1$ When adjoint scalars 
%%have large soft mass against $m_D$.  
%%
Alternatively, %as was pointed out in Ref.~\cite{Bertuzzo:2014bwa},
the adjoint Yukawa terms can relax 
the $D$-term suppression \cite{Bertuzzo:2014bwa,Diessner:2014ksa},
depending on the size and sign of a combination 
$\lambda_{ai}\mu_i/g_a m_{D_a}$.


Later we will consider the common value of 
$\suppressionD{D_1}=\suppressionD{D_2}
\left(=\suppressionD{D}\right)$
and treat it as a free parameter.
%%Typically we expect $\suppressionD{D_a}=1/2$ 
%%if $m_{D_a}^2=m_{\sigma_a}^2=m_{\pi_a}^2$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Pseudo moduli and pseudo Goldstino} %{{{
\label{subsec:pmoduli}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


The scalar potential in the $R$-symmetric Higgs sector takes the form
\begin{align} 
% V\ =\ V_F+V_{\mathrm{ad}}+V_D^{\mathrm{eff}}+V_{\mathrm{soft}} \ .
  V\ =\ V_F+V_A+V_D^{\mathrm{eff}}+V_{\mathrm{soft}} \ .
\label{eq:V}
\end{align}
Here $V_F$ and $V_A$  corresponds, respectively,
to the superpotential \eq{eq:W:Higgs} %\eq{eq:higgs:secter:superpot}
and \eq{eq:W:adjoint}, %\eq{eq:adjoint:Yukawa:superpot},
\begin{align} 
 V_F 
\ = \sum_{I=0,u,d}\abs{F_{Ri}}^2 + \sum_{i=u,d}\abs{F_{Hi}}^2
    \ , \qquad
% V_{{\rm ad}}
 V_A
\ =\ \sum_{a=1,2}\abs{F_{A_a}}^2
     \ ,
\nonumber
\end{align}
which reads,
%\rlap,\footnote{
%Here we have put adjoint scalar VEV's to zero
%by assuming large adjoint scalar masses.
%}
explicitly for the neutral components,
\begin{align} 
 V_F 
% &= \sum_{i=0,u,d}\abs{F_{Ri}}^2 + \sum_{i=u,d}\abs{F_{Hi}}^2
%\nonumber\\
 =&  \abs{f-\lambda H^0_u H^0_d}^2
   + \abs{\mu_d H^0_d}^2
   + \abs{\mu_u H^0_u}^2
%\nonumber\\
%  &{}
   + \abs{\mu_u R^0_u-\lambda  R_0 H^0_d}^2
   + \abs{\mu_d R^0_d-\lambda R_0 H^0_u}^2
    \,,
% \label{eq:VF:Higgs}\\
 \label{eq:V:RH}\\
% V_{{\rm ad}}
 V_A
 =& \sum_{a=1,2}
     \abs{%\sum_{i=u,d}
       \lambda_{ai} R_i^0 H_i^0}^2
\ =\ \left|\lambda ^u_S H^0_u R^0_u + \lambda ^d_S H^0_d R^0_d\right|^2
    +\left|\lambda ^u_T H^0_u R^0_u + \lambda ^d_T H^0_d R^0_d\right|^2
     \ .
% \label{eq:adjoint:pot}
 \label{eq:V:adjoint}
\end{align}
The last term $V_{\mathrm{soft}}$ stands for soft scalar masses,
\begin{align} 
V_{\mathrm{soft}}
 &=  \sum_{\varphi_i}m^2_{\varphi_i}\abs{\varphi_i}^2
     \ ,
 \label{eq:V:soft}
\end{align}
which can be induced from any $R$-invariant mediation of SUSY breaking
as in Refs.~\cite{Nelson:2002ca,Blechman:2009if,Kribs:2010md}.
Notice that
in \Eq{eq:V:RH},
we have put adjoint scalar VEV's to zero
by assuming large adjoint scalar masses.


%Let us focus on the $F$-term scalar potential
%by swithcing off soft SUSY breaking scalar massees
%and the gauge interactions,
%or equivalently, in the supersoft limit $\suppressionD{D}\rightarrow0$.
%Then the scalar potential
%corresponding to the superpotential \eq{eq:higgs:secter:superpot}
%corresponding to the superpotential \eq{eq:W:Higgs}
%has a flat direction,
%called pseudo moduli direction in the context of 
%spontaneout supersymmetry breaking~\cite{Intriligator:2007cp}.
%In the present paper,
%we shall discuss its impact on Higgs phenomenology
%and so let us elucidate it here.


%\paragraph{flat direction}


%The most characteristic feature of the present model 
%As we mentioned in Introduction,
As we mentioned in \S\ref{sec:introduction},
the model contains light degrees of freedom,
pseudo-moduli $\phi$ and pseudo-Goldstino $\psi$.
%One can most easily understand it by realizing that
One way to see their existence is to realize that
%the superpotential \eq{eq:higgs:secter:superpot} alone
the superpotential \eq{eq:W:Higgs} alone
defines a kind of O'Raifeartaigh model 
and that 
the corresponding  scalar potential $V_F$ has a flat direction,
called pseudo moduli direction in the context of 
spontaneous supersymmetry breaking~\cite{Intriligator:2007cp}.
In the present case,
it lies in the space of $R$-charged Higgs fields $R_{0,u,d}$
%$\left(R_0,\, R^0_u,\, R^0_d\right)$
and can be parametrized by polar angles as
\begin{align} 
 \left(R_0,R^0_u,R^0_d\right)
\ \sim\ %&= \phi
        \left(
        \cos\theta ,\  \sin\theta \cos\varphi , \ \sin\theta
        \sin\varphi
        \right)
 \ ,
 \label{eq:moduli:state}
\end{align}
where, %the polar angles are defined by
with $\VEV{H_u^0}=v_u=v\sin\beta$ and $\VEV{H_d^0}=v_d=v\cos\beta$,
\begin{align}
 \tan\theta
 &= \frac{\lambda v}{\mu}
  \equiv
  \lambda v\sqrt{
    \frac{\cos^2\beta}{\mu^2_u} + \frac{\sin^2\beta }{\mu^2_d}
    }
 \ ,\qquad
% \ ,\\
 \tan\varphi
 = \frac{\mu_u}{\mu_d}\tan\beta
% \ ,\\
% \frac{1}{\mu^2}
% &\equiv 
%    \frac{\cos^2\beta}{\mu^2_u} + \frac{\sin^2\beta }{\mu^2_d}
  \ . 
 \label{eq:angle:def}
\end{align}
\Eq{eq:moduli:state} is not a true flat direction, 
%but in the present case,
and is lifted by other terms in the scalar potential \eq{eq:V}.
To discuss its impact on Higgs phenomenology
is another purpose of the present paper.
%and so let us elucidate it here.


%The most characteristic feature of the present model 
%is the presence of light degrees of freedom,
%pseudo-moduli $\phi$ and pseudo-Goldstino $\psi$.
%One can most easily understand it
%by focusing the $F$-term scalar potential $V_F$
%corresponding to the superpotential \eq{eq:higgs:secter:superpot},
%corresponding to the superpotential \eq{eq:W:Higgs},
%which has a flat direction,
%called pseudo moduli direction in the context of 
%spontaneout supersymmetry breaking~\cite{Intriligator:2007cp}.
%This is not a true flat direction, but in the present model,
%it is lifted by other terms in the scalar potential \eq{eq:V}.
%It is another purpose of the present paper
%to discuss its impact on Higgs phenomenology,
%and so let us elucidate it here.


%\paragraph{pgoldstino}


Let us first discuss the pseudo-Goldstino.
The present model contains nine components of neutralinos:
two gauginos $\lambda_{a=1,2}^0$
and three $R$-charged Higgsinos $\wt{R}_{0,u,d}^0$
of $R$-charge $+1$,
and two Higgsinos $\wt{H}_{u,d}^0$
and two adjoint fermions $\chi_{a=1,2}^0$
of $R$-charge $-1$.
Among them,
we are interested in the lightest mass eigenstate $\psi$,
which is called ``pseudo-Goldstino''.
It can get a mass only from 
explicit $R$-symmetry breaking \cite{Bertolini:2011tw,Morita:2012kh},
which we can neglect for the present purpose
and so we treat it as a massless fermion.
%
%[We treat it as massless
%since we are neglecting small $R$-breaking effects.]
%
In the absence of the adjoint Yukawa terms 
\eq{eq:W:adjoint}, %\eq{eq:adjoint:Yukawa:superpot},
the pseudo-Goldstino is a mixture of $\wt{R}_{I=0,u,d}^0$;
in terms of the polar angles \eq{eq:angle:def},
\begin{align} 
% \left(\tilde{R}_0,\tilde{R}^0_u,\tilde{R}^0_d\right)
% &= \psi\left(
%        \cos\theta ,\ \sin\theta \cos\varphi , \ \sin\theta \sin\varphi
%        \right)\ ,
%\\
\psi
 &= \wt{R}_0\cos\theta
   +\left(\wt{R}^0_u\cos\varphi+\wt{R}^0_d\sin\varphi
    \right)\sin\theta
\ \equiv
    \sum_{I=0,u,d} U_{\psi I}\wt{R}^0_I 
    \ .
 \label{eq:goldstino:state}
\end{align}
The angle $\theta$ is the mixing angle between 
$SU(2)$-singlet $\wt{R}_0$ and doublets $\wt{R}_{u,d}^0$.
Note that 
the parameter $\mu$ defined in \Eq{eq:angle:def}
can be regarded as a representative scale of Higgsino masses.


In passing,
it is interesting to note that
the pseudo-Goldstino $\psi$ can have nonzero gaugino components 
in some cases.
%First, it has tiny gaugino components after 
%the inclusion of explicit $R$-symmetry breaking \cite{Morita:2012kh}.
First, the inclusion of explicit $R$-symmetry breaking
can give a tiny gaugino components \cite{Morita:2012kh}.
In addition,
the adjoint Yukawa couplings $\lambda_{ai}$
%in \Eq{eq:adjoint:Yukawa:superpot} give 
in \Eq{eq:W:adjoint} give 
%after EW symmetry breaking 
mixing terms between the $R$-charged Higgsinos $\wt{R}_{i=u,d}$ 
and the adjoint fermions $\chi_{a=1,2}$,
%($\chi_1^0=\wt{S}$ and $\chi_2^0=\wt{T}^0$),
\begin{align} 
%{}-\mathcal{L}_{\psi, \tilde{A}}
{}-\mathcal{L}_{\psi \chi}
\ = \sum_{a=1,2}\sum_{i=u,d}  \lambda_{ai}v_i\wt{R}_i^0\chi_a^0
\ =\ \lambda^u_S v_u \wt{R}^0_u \wt{S}   +  \lambda^d_S v_d \wt{R}^0_d \wt{S}
    +\lambda^u_T v_u \wt{R}^0_u \wt{T}^0 + \lambda^d_T v_d \wt{R}^0_d \wt{T}^0
     \ .
\end{align}
where $\chi_1^0=\wt{S}$ and $\chi_2^0=\wt{T}^0$.
%In the presence of these mixing terms,
Diagonalizing it gives %the pseudo-goldstino 
$\psi$ a gaugino component of $\order{\lambda_{ai}v_i/m_D}$. 
%Note that the gaugino component of the pseudo-Goldstino is small 
%if the adjoint Yukawa couplings are small.
%[We will mainly neglect it
%when we discuss phenomenology of pseudo-goldstino.]
Although this can be neglected in our later analysis,
it may be relevant for other purposes,
\eg, cosmological implications of the pseudo-Goldstino.


%\paragraph{pmoduli}


Next we turn to the pseudo-moduli $\phi$,
the lightest mass eigenstate in the $R$-charged scalars $R_{0,u,d}^0$.
Essentially it is a fluctuation 
along the 'flat' direction \eq{eq:moduli:state},
but in the presence of soft terms 
as well as $D$-terms and adjoint Yukawa terms,
it can deviate from that direction.
That is, if we write the pseudo-moduli state as
\begin{align}
\phi
\ \equiv
    \sum_{I=0,u,d} U_{\phi I} R^0_I
    \ ,
 \label{eq:pmoduli:state}
\end{align}
the mixing angles $U_{\phi I}$ are in general
different from $U_{\psi I}$ in \Eq{eq:goldstino:state}.
Accordingly,
%the pseudo-moduli gets a mass mainly from the soft scalar masses
%of the $R$-charged scalars $R_{0,u,d}$.
important for the pseudo-moduli mass $m^2_{\phi}$
are the soft scalar masses of the $R$-charged scalars $R_{0,u,d}$.
Later we will consider the case in which 
the doublets $R_{u,d}$ have a common soft mass $m^2_{R}$,
while the singlet $R_0$ can have a different mass $m^2_{R_0}$,
\begin{align}
V_{\mathrm{soft},R}
\ =\ m^2_{R_0}\abs{R_0}^2
    +m^2_{R}\sum_{i=u,d}\abs{R_i}^2
     \ .
\label{eq:V:soft:R}
\end{align}
%where $m^2_{R_0}$ is the soft mass of the singlet $R_0$
%and $m^2_{R}$ is the common soft mass of the doublets $R_{u,d}$.
When $m_{R_0}^2=m_R^2$,
the pseudo-moduli can be made heavy, $m^2_\phi=m^2_\psi+m^2_R$,
with the same mixing angles $U_{\phi I}=U_{\psi I}$,
as in the pseudo-Goldstino state \eq{eq:goldstino:state}.


It may be plausible that
the singlet $R_0$ does not have a soft mass
as is often the case in gauge mediation of SUSY breaking.
In this case, $m_{R_0}^2=0$,
the pseudo-moduli gets a mass $m^2_\phi$ 
through the mixing to the doublets $R_{u,d}$,
so that $m^2_\phi$ shows some interesting behaviour.
For later reference, let us elucidate the $m^2_{R_0}=0$ case
in the isospin symmetric case, \ie,
by assuming $\tan\beta=1$ and $U_{\phi u}=U_{\phi d}$
so that $\phi$ lies along
$D$-flat direction of $R_{u,d}$.
%When the Higgsino mass parameter $\mu$ is much greater than $m_R$,
When the soft mass $m_R$ can be regarded as a small perturbation,
%the Higgsino mass parameter $\mu$ is much greater than $m_R$,
the mass eigenvalue behaves like
\begin{align}
m^2_\phi
\ \sim\ m^2_R\sin^2\theta
\ \sim\ m^2_R\,\frac{\lambda^2 v^2}{\lambda^2 v^2+\mu^2}
        \ .
\label{eq:moduli:mass:mu:small}
\end{align}
Conversely,
when the soft mass parameter $m_R$ as well as $\mu$ 
are much greater than $\lambda v$,
the singlet $R_0$ dominates the pseudo-moduli,
so that its mass eigenvalue behaves like
\begin{align}
m^2_\phi
\ \sim\ \lambda^2 v^2
        \frac{m^2_R}{m^2_R+\mu^2}
%\ \sim\ \lambda^2 v^2
%       -\frac{\left(\lambda v \mu\right)^2}{m^2_R}
%       +\cdots
        \ .
\label{eq:moduli:mass:mu:large}
\end{align}
In these cases,
the pseudo-moduli $\phi$ can be well lighter than
the SM-like Higgs boson.
We will further examine the properties of the pseudo-moduli
in \S{\ref{sec:decay}}.
%where we will take $m_{R_0}^2/m_R^2=\{0,\,0.2,\,0.5\}$
%as a representative case.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%





==> v2_changelog/sec3_triviality20160107a.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Gauge Coupling Unification and Lightest Higgs Mass}
\section{Perturbative Unification and Lightest Higgs Mass}
%\label{sec:higgs:mass}
\label{sec:triviality}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


In this section, we examine gauge coupling unification 
and triviality %(perturbativity) 
bound on the lightest Higgs mass 
in the present $R$-symmetric model.
Since the model is a kind of 
singlet extension of the minimal $R$-symmetric model,
the most important for reproducing the Higgs mass of $125\nunits{GeV}$
is the singlet Yukawa interaction $\lambda R_0 H_u H_d$,
which is subject 
to the triviality (perturbativity) constraint\,\footnote{
An alternative possibility is 
to implement the fat Higgs idea \cite{Harnik:2003rs}
in an $R$-symmetric setup,
but we do not pursue it here.
}
as in the conventional singlet extensions of the MSSM.
To discuss the triviality bound,
we need a ``UV completion'' of Dirac gaugino model.
Here we adopt a minimal model 
that is consistent with perturbative unification,
although we do not discuss its embedding into
any concrete realizations of grand unified theories.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Gauge Coupling Unification} %{{{
\label{subsec:unification}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Gauge coupling unification is not automatic
in models with Dirac gaugino
since we introduce 
adjoint chiral multiplets $\mathcal{A}_{a=3,2}$ 
which contribute to gauge beta functions $\beta_{g_a}$.
In addition, $R$-charged Higgs doublets $R_{u,d}$
are introduced.
As was noted 
by many authors \cite{Fox:2002bu,Kribs:2007ac,Benakli:2014cia}, 
the simplest way to recover the unification 
is to add two pairs of $SU(3)\times SU(2)$--singlets
with $U(1)_Y$--charge $\pm 1$, $\left(E^c_{4,5},\wb{E}^c_{4,5}\right)$,
with a mass term $\ME E^c_i \wb{E}^c_i$ ($i=4,5$).
For definiteness,
we refer to these `bachelor'' states\,\footnote{
Phenomenological implications of these extra ``leptons''
would be interesting but are beyond the scope of the present paper.
}
 as ``extra leptons''.
[See Table~\ref{tab:contents}.]
The resultant extra matter content is 
%essentially the same as implied from 
consistent with $SU(3)_c\times SU(3)_L\times SU(3)_R$ 
trinification \cite{trinification1,trinification2}:
the extra matter fields,
$\mathcal{A}_a$, $R_{u,d}$ as well as
the `bachelor'' $\left(E^c_{4,5},\wb{E}^c_{4,5}\right)$,
can be embedded into an adjoint representation of $SU(3)^3$,
modulo the SM singlets. 
Accordingly
one-loop coefficients of gauge beta functions,
$\left(16\pi^2\right)dg_a/dt=b_a g_a^3$ ($a=3,2,1$), 
are shifted by the same amount, $b_a=b_a^{\mathrm{MSSM}}+3$,
where $g_1=\sqrt{5/3}\,g_Y$.


Note that
the extra contribution to gauge beta functions
makes the UV gauge couplings stronger than those in the MSSM.
This fact is important
since it relaxes triviality bound for the Higgs mass,
as we shall see shortly.
In this respect, 
%we notee that 
the present setup is the minimal one:
adding more fields would make the gauge couplings stronger
at UV and further relax the triviality bound.
[See Ref.~\cite{Kakizaki:2013eba} 
for another nontrivial choice of extra matter content.]


At one-loop level, gauge coupling unification is preserved,
as is depicted in Fig.~\ref{fig:GUT:1-loop},
if all the extra particles beyond the SM ones
have the common mass $\MS$ around TeV range.
Here the extra particles include
Dirac gauginos and scalar partners, 
heavier Higgses and Higgsinos, and the extra leptons, 
%$R$-charged Higgses, and the extra leptons, 
in addition to other SUSY particles.


\begin{figure}[btp]
  \begin{center}
		\includegraphics[scale=0.5]{fig_gauge_1-loop_light.eps}
  \end{center}
\caption{
One-loop running of gauge couplings
in the present model (thick solid)
is compared with those in the MSSM (thin solid)
and the MSSM with adjoint chiral fields added (dashed).
%All the particles beyond the SM ones are assumed to decouple
%at a single scale $\MS=1\nunits{TeV}$.
%[Dashed lines are $\alpha_{2,1}^{-1}$ in the MSSM with 
%only adjoint chiral fields added.]
The vertical axis is $\alpha_a^{-1}=4\pi/g_a^2$
and horizontal axis is the renormalization scale $Q$.
%The vertical and horizontal axises are
%$\alpha_a^{-1}=4\pi/g_a^2$ and 
%the renormalization scale $Q$, respectively.
}
\label{fig:GUT:1-loop}
\end{figure}


Of course,
gauge coupling unification is still nontrivial 
when two-loop RGE's are used
and/or masses of the extra particles are not degenerate.
%[The relevant RGE's are summarized in \S{\ref{sec:RGanalysis}}.]
In the present work, however,
we do not intend to examine the precision of unification
to its full details, \eg, 
by taking spectrum of extra particles into account,
as was done in Ref.~\cite{Benakli:2014cia}
for the constrained minimal Dirac Gaugino SUSY SM (CMDGSSM);
Instead, we give a few examples in which unification is achieved
to the extent that is enough for estimating the bound for the Higgs mass.
%The relevant RGE's are summarized in \S{\ref{sec:RGanalysis}}.


In the following RG analysis,
we use two-loop RGE's summarized in \S{\ref{sec:RGanalysis}}.
%we will make a simplifying assumption that
In addition, we will assume that
%the same is true, \ie,
%% except in the cases explicitly stated:
%%%In fact we will consider the followoing cases:
all the extra particles are approximately degenerate around 
the scale $\MS=1\nunits{TeV}$ or $2\nunits{TeV}$,
except that
\begin{enumerate}
\item[(i)]
the extra lepton mass $\ME$ can be different from $\MS$,
\item[(ii)]
the $SU(3)$ or $SU(2)$ Dirac mass threshold,
$M_{D_3}$ or $M_{D_2}$, defined by \Eq{eq:MD:def},
can be different from $\MS$.
\end{enumerate}
%Notice that
Unlike the heavy Majorana gluino case,
a heavy Dirac gluino does not necessarily imply heavy squarks,
thanks to ``supersoftness'' of soft scalar masses.
This partially justifies our simplifying assumption as above.


%Actually RG analysis including soft parameters
%was given in Ref.~\cite{Benakli:2014cia}
%for the constrained minimal Dirac Gaugino SUSY SM (CMDGSSM).
%The GUT boundary condition for the Dirac gaugino massess
%would imply the specific mass ratios,



%It should be noted that
%one can in principle recover the unification
%by tuning the bachelor mass $\ME$ in. 
%[See below, however.]
%So the unification is not a prediction at all.
%To discuss the triviality bound on the Higgs mass, however,
%we need a UV extension of Dirac gaugino model.
%To this end, the present setup is the minimal one:
%adding more fields would make the gauge coupling stronger
%at UV and thus relax the triviality bound.
%Figure~\ref{fig:GUT:1-loop} shows one-loop running of the gauge couplings
%in the MSSM with/without the  adjoint chiral fields
%% (CMDGSSM\cite{Benakli:2014cia}) 
%and the present model. 


%Notice that
Note that
two-loop RG evolution of gauge couplings
depends on the singlet, %Yukawa $\lambda$
the adjoint %Yukawa $\lambda_{ai}$
and the top Yukawa couplings,
$\lambda$, $\lambda_{ai}$ and $y_t$.
%[The relevant RGE's are given in \S{\ref{sec:RGE:ad:1-loop}}.]
Therefore the precision of unification
can be discussed only after
the correct value of the lightest Higgs mass is reproduced.
It also depends on the suppression factor $\suppressionD{D}$
for $D$-term quartic
since $\suppressionD{D}=0$, for instance, requires a larger $\lambda$,
which implies a larger two-loop effect on gauge runnings.
%[In the above examples, we have taken these effects into account.]
Being so,
further details about gauge coupling unification
at two-loop level are presented in \S{\ref{sec:unification}}.


%In calculating the upper bound,
%we do not require the unification at two-loop level.
%ftso we just calculate it by assuming the single mass threshold.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Triviality Bound on Singlet Yukawa Coupling}
\label{subsec:triviality}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Having discussed a UV completion of the model,
we now examine the triviality bound,
by requiring that
no coupling constant exceeds a perturbativity bound $\sqrt{4\pi}$ 
up to UV cutoff $\Lambda$,
for which we consider two cases:
lower cutoff $2.0\times 10^{16}\nunits{GeV}$ 
and higher one $1.0\times 10^{17}\nunits{GeV}$.


First let us focus on the case 
without the adjoint Yukawa couplings $\lambda_{ai}$.
Then the quantitative behaviour can be seen from one-loop RGE's 
for $\lambda$ and
the top Yukawa %coupling 
$y_t$, % and the singlet Yukawa coupling 
\begin{align} 
 \frac{dy_t}{dt}
\ =&\ \frac{y_t}{16\pi^2}
    \left(
       6y^2_t + \lambda^2
       -\frac{16}{3}g^2_3 - 3g^2_2 - \frac{13}{9}g^2_Y
    \right)
    \ ,
    \label{eq:yt RGE}\\
 \frac{d\lambda}{dt}
\ =&\ \frac{\lambda}{16\pi^2}\,
    \Bigl(
        4\lambda^2 + 3y^2_t - 3g^2_2 - g^2_Y
    \Bigr)
    \ ,
\label{eq:lambda:RGE}
\end{align}
where $g_Y=\sqrt{3/5}g_1$.
As we mentioned,
the UV gauge coupling constants in the present model
are larger than those in the MSSM or its singlet extensions.
%, like the NMSSM or the nMSSM.
It follows that
the triviality %(perturbativity) 
bound for %the singlet Yukawa coupling 
$\lambda$ as well as $y_t$ is relaxed.


Figure~\ref{fig:cont:pert} shows the upper bound 
that we obtain by using two-loop RGE's. 
In the left panel,
the present case is compared with
the nMSSM-like case whose matter content is 
the same as in the singlet extension of the MSSM,
but without the cubic coupling $\kappa$ of the singlet.
Numerically,
for $\MS=1\nunits{TeV}$ and $\tan\beta=2$ ($y_t=0.95$),
the upper bound on $\lambda\fun{\MS}$
from $\Lambda=2.0\times 10^{16}\nunits{GeV}$ is $0.775$,
which is improved from $0.696$ in the nMSSM-like case,
and becomes sightly reduced to $0.762$ 
for $\Lambda=1.0\times 10^{17}\nunits{GeV}$.
%See Table.~\ref{tab:lambda:critical} for numerital values.


\begin{figure}[tbp]
  \begin{tabular}{lr}
 \begin{minipage}{0.45\hsize}
    \begin{center}
    \includegraphics[scale=0.6]{fig_lambda2-cr_pre-nMSSM_light.eps}
     \end{center}
      \end{minipage}
      \hspace{3mm}
      \begin{minipage}{0.45\hsize}
       \begin{center}
      \includegraphics[scale=0.6]{fig_lambda2-cr_adjoint_light.eps}
  \end{center}
	\end{minipage}
 \end{tabular}
\caption{
Triviality bound on squared couplings $y^2_t$ and $\lambda^2$.
%evaluated at $\MS=1\nunits{TeV}$. 
In the left, 
the upper solid (lower dashed) lines correspond to
the present model (nMSSM), respectively. 
The bounds are obtained
from perturbativity up to $2.0\times 10^{16}\nunits{GeV}$,
except for the thin line 
%for which we require up to $1.0\times 10^{17}\nunits{GeV}$.
for $1.0\times 10^{17}\nunits{GeV}$.
In the right, 
the blue solid and black dashed lines correspond to
$\lambdaad=0$ and 
%$\lambdaad}=
$\{0.2,\, 0.3,\, 0.4,\, 0.5\}$ 
from the top.
In each figure, 
all the couplings are evaluated at $\MS=1\nunits{TeV}$,
and the vertical line corresponds to $\tan\beta=2$.
 }
%\label{fig:critical:ad}
\label{fig:cont:pert}
\end{figure}


We also show in the right panel of Fig.~\ref{fig:cont:pert}
how the upper bound on $\lambda$ becomes tight
when the adjoint Yukawa couplings $\lambda_{ai}$ become large.
For definiteness,
we input a common value $\lambdaad$ for $\lambda_{ai}$
at the scale $\MS=1\nunits{TeV}$ or $2\nunits{TeV}$.
Numerical values are shown %for $\tan\beta=2$
in Table~\ref{tab:lambda:critical}.
%We see that sizable adjoint Yukawa couplings are not favored
%if the Higgs mass of $125\nunits{GeV}$ 
%is to be reproduced by the singlet Yukawa $\lambda$.


\input table2_bound20151207a.tex


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Higgs Mass in Models without Adjoint Yukawa Couplings}
\subsection{Triviality Bound on Higgs Mass}
\label{subsec:Higgsmass}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Now, we examine the mass of the lightest Higgs boson
and calculate its upper bound.
Here we adopt the RG approach,
and calculate the lightest Higgs mass 
by matching the present $R$-symmetric SUSY model
to a low-energy effective theory at the single scale $\MS$.
To be more precise,
starting from the input parameters summarized 
in \S{\ref{sec:inputs}},
we evolve the effective theory couplings
from the top mass scale to the matching scale $\MS$,
at which we switch to the $R$-symmetric SUSY model.
At this step, we input a value of $\tan\beta=\VEV{H_u^0}/\VEV{H_d^0}$ 
to match the top Yukawa coupling.
Then we evolve the SUSY couplings to UV region
and require the perturbativity as before.
%that no coupling exceeds 
%a perturbativity bound $\sqrt{4\pi}$ 
%below a unification scale. 
%As the unification scale, we consider two cases; 
%$2\times 10^{16}\nunits{GeV}$ and $1\times 10^{17}\nunits{GeV}$.


As for the matching scale,
we take $\MS=1\nunits{TeV}$ or $2\nunits{TeV}$.
Notice that
this corresponds to a relatively low SUSY scale,
which is still consistent with the LHC bounds
thanks to ``supersafeness'' of Dirac gaugino scenario
\cite{Nojiri:2007jm,Heikinheimo:2011fk,Kribs:2012gx}.
At the same time, however,
it is quite nontrivial to reproduce the $125\nunits{GeV}$ Higgs
since 
radiative corrections from the top-stop sector are not so large;
$A$-terms are forbidden by the $R$-symmetry.


%We use two-loop RGE's
%$\beta_i=\beta_i^{(1)}/\left(16\pi^2\right)
%+\beta_i^{(2)}/\left(16\pi^2\right)^2$,
%where some one-loop parts are shown below
%while two-loop parts are shown for completeness in App. 


%\paragraph{Matching to SM}


As for the low-energy effective theory,
we mainly consider the minimal SM model
by taking the decoupling limit of heavier Higgs mass eigenstates.
[We will also examine the matching
to the SM coupled with a light pseudo-moduli
in \S{\ref{subsec:match2pmoduli}}.]
%in the next subsection.]
Then the matching condition to the quartic Higgs potential, 
$V_{\textrm{eff}}\fun{H}=\left(\lambda_H/2\right)\abs{H}^4$,
is given by
\begin{align} 
% V_{\textrm{eff}}\fun{H}
% &=\ \frac{1}{2}\,\lambda_H\abs{H}^4
%     \ , 
%\nonumber\\
 \lambda_H\fun{\MS}
% &=  \frac{1}{2}\,\lambda^2(\MS) \sin^2\left(2\beta\right) 
%  +  \frac{1}{4}\,\suppressionD{D}g^2_Z(\MS)\cos^2\left(2\beta\right)
 &=\  \frac{1}{2}\,\lambda^2\fun{\MS} \sin^2{2\beta}
    + \frac{1}{4}\,\suppressionD{D\,}g^2_Z\fun{\MS}\cos^2{2\beta}
      \ ,
\label{eq:matching:SM}
\end{align}
where $g_Z^2=g_Y^2+g_2^2$ and 
$\suppressionD{D}$ is the (common) suppression factor of $D$-term 
defined in \Eq{eq:Dterm:pot}.


Figure~\ref{fig:Higgs:mass:bound} summarizes our results,
showing the upper bound on the lightest Higgs mass 
as a function of $\tan\beta$,
for various cases.
%The right figures correspond to the matching
%to the SM with a pseudo-moduli included,
%about which we defer discussion to the next subsection.
%
%The matching to the minimal SM is shown in the left figures.
The left panel corresponds to the case
without adjoint Yukawa couplings.
We see that 
$125\nunits{GeV}$ Higgs mass can well be reproduced
at a small value of $\tan\beta$ around $2$--$4$.
It should be emphasized that this is possible
even without the $SU(2)\times U(1)$ quartic $D$-terms 
and with the SUSY scale as low as $1\nunits{TeV}$.


The right panel shows to what extent
the adjoint Yukawa couplings $\lambda_{ai}$ reduce the upper bounds
in the case of a common value $\lambdaad=0.3$.
We see that
$125\nunits{GeV}$ Higgs mass can be reproduced,
but requires a larger SUSY scale ($\MS=2\nunits{TeV}$)
or non-zero $D$-term ($\suppress{D}\neq0$).


\begin{figure}[tbp]
 \begin{tabular}{lr}
  \begin{minipage}{0.45\hsize}
    \begin{center}
      \includegraphics[scale=0.8]{fig_mh-tanb_MS2_SM.eps}
    \end{center}
  \end{minipage}
  \hspace{3mm}
  \begin{minipage}{0.45\hsize}
    \begin{center}
%#	\includegraphics[scale=0.8]{fig_mh-tanb_MS2_CSSM.eps}
	\includegraphics[scale=0.8]{fig_mh-tanb_MS2_lamad03.eps}
    \end{center}
  \end{minipage}
 \end{tabular}
\begin{tabular}{lr}
  \begin{minipage}{0.45\hsize}
    \begin{center}
      \includegraphics[scale=0.8]{fig_mh-tanb_MS1_SM.eps}
    \end{center}
  \end{minipage}
  \hspace{3mm}
  \begin{minipage}{0.45\hsize}
    \begin{center}
%#	\includegraphics[scale=0.8]{fig_mh-tanb_MS1_CSSM.eps}
	\includegraphics[scale=0.8]{fig_mh-tanb_MS1_lamad03.eps}
    \end{center}
  \end{minipage}
 \end{tabular}
\caption{
Upper bounds of the lightest Higgs mass as a function of $\tan\beta$. 
The upper (lower) figures correspond to the SUSY scale
$\MS=2\nunits{TeV}$ ($\MS=1\nunits{TeV}$), respectively.
In each figure, upper blue (lower red) lines correspond to 
the unsuppressed $D$-term $\suppress{D}=1$ 
(completely suppressed $D$-term $\suppress{D}=0$), respectively.
In the left panel,
we tale $\lambdaad=0$, and
the dashed line corresponds to the nMSSM-like case.
The bounds are obtained
from perturbativity up to $\Lambda=2.0\times 10^{16}\nunits{GeV}$,
except for the thin lines 
corresponding to $\Lambda=1.0\times 10^{17}\nunits{GeV}$.
In the right panel,
we compare the $\lambdaad=0.3$ case (solid lines)
with the $\lambdaad=0$ case (dashed lines).
         }
\label{fig:Higgs:mass:bound}
\end{figure} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Remarks}
\label{subsec:remarks}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



Some remarks are in order here.


The above result is to be compared with the nMSSM-like case, 
which typically requires a higher SUSY scale or sizable stop mixing
\cite{Ellwanger:2012ke,Ishikawa:2014owa}.
We also note that,
unlike the existing singlet extension of the MSSM,
the NMSSM or nMSSM or PQ-NMSSM \cite{Jeong:2012ma}
in which the singlet-doublet mixing can raise
the mass of the SM-like Higgs boson,
the approximate $R$-symmetry forbids such mixing
between our singlet state $R_0$ and the SM-like Higgs boson.


Another remark is that
the calculated Higgs mass may be a bit underestimated
especially for a low SUSY scale.
Actually improved two-loop calculations show
the SM-like Higgs mass receives a significant correction
in the NMSSM \cite{Goodsell:2014pla}
if the singlet is light,
and also in the MRSSM \cite{Diessner:2015yna}.
Nevertheless,
it is also clear that
the present model gives a sufficiently large improvement.



%In this respect,
%a worry is that our estimate here might overestimate
%the Higgs mass
%if there is a light scalar that strongly coupled
%to the SM-like Higgs boson below the matching scale $\MS$.
%So we shall examine this point in the next subsection.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Note on Adjoint Yukawa Couplings}
%\label{subsec:adjoint}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Finally let us briefly discuss to what extent
the adjoint Yukawa couplings are allowed
for realizing $125\nunits{GeV}$ Higgs mass.
Figure~\ref{fig:Higgs:mass:contour:ad} shows 
contours of the Higgs masses
in the space of $\left(\tan\beta,\lambdaad\right)$,
for a larger $\MS=2\nunits{TeV}$.
As is seen from the left panel,
if we input a common value of adjoint Yukawa couplings 
$\lambda^{u,d}_{S,T} = \lambdaad$ at the scale $\MS$,
its upper limit is around $ \lambdaad \sim 0.3\hbox{--}0.4$
depending on the $D$-term suppression factor $\suppress{D}$.
The right panel also shows that
compared with the left,
$\lambda_{T}$ can be about $15\,\%$ larger if $\lambda^{u,d}_{S}=0$,
while 
$\lambda_{S}$ can be about $38\,\%$ larger if $\lambda^{u,d}_{T}=0$.



\begin{figure}[tbp]
 \begin{tabular}{lr}
  \begin{minipage}{0.45\hsize}
   \begin{center}
     \includegraphics[scale=0.8]{fig_mhcont_lamad_MS2.eps} 
   \end{center}
  \end{minipage}
  \hspace{4mm}
  \begin{minipage}{0.45\hsize}
   \begin{center}
     \includegraphics[scale=0.8]{fig_mhcont_lamad-oneside_MS2.eps}
   \end{center}
  \end{minipage}
 \end{tabular}
\caption{
The upper bounds of adjoint Yukawa couplings 
%as a function of $\tan\beta$ 
for $\MS=2\nunits{TeV}$ case.
In the left, %where $\lambda ^{u,d}_{S,T}=\lambda _{{\rm ad}}$,
the upper bounds %for $\lambdaad$
corresponding to the Higgs mass 
%$120$, $125.7$ and $130\nunits{GeV}$
$120$, $125$ and $130\nunits{GeV}$
are shown from the top, 
by blue dots ($\suppress{D}=1$) 
and red dots ($\suppress{D}=0$), respectively.
%
In the right ($\suppress{D}=0.5$),
the contour of the Higgs mass $125\nunits{GeV}$
are shown for three cases 
$(\lambda^{u,d}_S,\lambda^{u,d}_T)
=\left(\lambdaad,0\right)$,
$\left(0,\lambdaad\right)$ and
$\left(\lambdaad,\lambdaad\right)$,
from the top by black, red and blue dots, respectively.
%The parameters are $\MS=2\nunits{TeV}$ and $\suppressionD{D}=0.5$. 
 }
%\label{fig:mhcont:ad:an}
\label{fig:Higgs:mass:contour:ad}
\end{figure}


Notice that
$\lambda=0$ corresponds to
the minimal $R$-symmetric model (MRSSM),
where 
the Higgs mass can be reproduced in a large $\tan\beta$ region.
In this sense,
there are two possibilities in $R$-symmetric models:
\begin{enumerate}
\item[(i)]
large $\tan\beta$ solution:
the $125\nunits{GeV}$ Higgs can %marginally 
be reproduced by the large adjoint Yukawa couplings
and corresponding radiative corrections.
\item[(ii)]
small $\tan\beta$ solution:
the $125\nunits{GeV}$ Higgs can easily be reproduced
by the large singlet Yukawa coupling
(and small adjoint couplings).
\end{enumerate}
The former requires nontrivial mass splitting
within $R$-charged Higgses and $SU(2)\times U(1)$ adjoints
so that the large adjoint coupling(s)
can play a similar role as the top Yukawa $y_t$ in the MSSM.
In our treatment,
such effects are not incorporated
since we are treating the SUSY spectrum
as a single mass threshold.


%{{{ Matching to SM with pmoduli
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Matching to the SM coupled with Pseudo-Moduli}
\label{subsec:match2pmoduli}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%\paragraph{Matching to SM with pmoduli}


As we described in \S{\ref{subsec:pmoduli}},
the present model contains
a light degree of freedom, pseudo-moduli $\phi$, 
which is a complex scalar and can couple 
to the SM-like Higgs field.
%%%\rlap.\footnote{
%%%[memo]: --- to be modified ---
%%%We just assume that
%%%the inclusion of the second and third lightest mass eigenstates
%%%does not modify the present result so much.
%%%This is actually the case when
%%%the lightest state is approximately given by
%%%the singlet $R_0$ and the others are given by the doublets $R_{u,d}$,
%%%since the latter does not have a large quartic coupling 
%%%to $H_{u,d}$ from $F$-term. 
%%%$D$-term is small in an interesting region of small $\tan\beta$.
%%%}
Therefore it can affect the mass of the SM-like Higgs.
To estimate this effect,
we consider the effective theory
that contain the SM and the pseudo-moduli,
\begin{align} 
 V_{\rm{eff}}\fun{H,\phi}
 &= \frac{1}{2}\,\lambda_H \abs{H}^4 
  + \lambda_{\phi H} \abs{\phi}^2 \abs{H}^2
  + \lambda_\phi \abs{\phi}^4
    \ .
 \label{eq:CSSM}
\end{align}
It is not clear to us which field
should be identified with the moduli field $\phi$ 
in a symmetric phase of the effective theory
since 
the singlet $R_0$ can not mix with the doublets $R_{u,d}$
before the EWSB.
Recall from \S{\ref{subsec:pmoduli}}, however,
that the pseudo-moduli $\phi$ is light
especially when the Higgsino mass parameter $\mu$ is large 
and the soft mass $m_R$ is small.
In this situation,
the singlet scalar $R_0$ dominates the pseudo-moduli mass eigenstate.
So we construct the low-energy effective theory
by identifying the pseudo-moduli $\phi$ with the singlet $R_0$.


To be specific, let us assume $\mu=\order{\MS}$
and integrate out the heavy doublet fields $R_{u,d}$.
This leads to the tree-level matching condition 
\eq{eq:matching:SM} supplemented by
\begin{align} 
% \lambda_H(\MS)
% &=  \frac{1}{2}\,\lambda^2(\MS) \sin^2\left(2\beta\right) 
%  +  \frac{1}{4}\,\suppressionD{D}g^2_Z(\MS)\cos^2\left(2\beta\right)
%     \ ,
%\\
 \lambda_{\phi H}(\MS) 
 &=  \suppressionD{R\,}
     \lambda^2(\MS)
     \ , \qquad 
 \lambda_\phi(\MS) = 0
     \ ,
\label{eq:matching:portal}
\\
\suppressionD{R}
 &\equiv
      \frac{m^2_{R_u} }{\mu^2_u + m^2_{R_u} } \cos^2\beta
    + \frac{m^2_{R_d} }{\mu^2_d + m^2_{R_d} } \sin^2\beta
    \ ,
\label{eq:suppressionR}
\end{align}
%Here we have neglected possible threshold effects
%of other mass eigenstates of $R$-charged Higgs fields.
where $m_{R_{u,d}}$ are the soft mass of $R_{u,d}$.
Here we have introduced a factor $\suppress{R}$
which represents a suppression of the ``portal'' coupling
$\lambda_{\phi H}$ at the matching scale.
This is a kind of non-decoupling effect
proportional to soft SUSY breaking parameters,
$\suppress{R}\rightarrow m^2_R/\left(\mu^2+m^2_R\right)$
for $\mu_u=\mu_d$ and $m^2_{R_u}=m^2_{R_d}$,
which is small if $m_R\ll\mu$.
On the other hand,
it can be of $\order{1}$ if $m_R\gg \mu$.
Even in this case,
\Eq{eq:moduli:mass:mu:large} shows that
the $\phi$ can remain light if $m_{R_0}=0$.
Then the ``portal'' coupling  $\lambda_{\phi H}$ is quite large at $\MS$.


For definiteness, we examine the extreme case
in which the pseudo-moduli is lighter than the SM-like Higgs boson.
Then we evolve the couplings in the effective theory \eq{eq:CSSM}
from $\MS$ down to the Higgs mass scale,
by using two-loop RGE's shown in \S{\ref{sec:RGE:CSSM}}.
Here we show one-loop parts,
which already contain the most important term:
\begin{align} 
 \beta_{\lambda_H}^{(1)}
 &=    \left. \beta_{\lambda_H}^{(1)}\right\vert_{\mathrm{SM}}
    +2 \lambda_{\phi H}^{2}   
    \ , 
\label{eq:RGE:lambdaH:oneloop}\\
 \beta_{\lambda_{\phi H}}^{(1)}
 &=  \lambda_{\phi H}
     \left(  6 \lambda_H + 4 \lambda_{\phi H}+ 2 \lambda_{\phi}   
	 + 6 y^2_t 	 -\frac{9}{2} g_{2}^{2} -\frac{15}{2}
         g_{Y}^{2} 
     \right)
     \ ,\\
 \beta_{\lambda_\phi}^{(1)}
 &=  8 \lambda_{\phi H}^{2}+ 5 \lambda_{\phi}^{2}
     \ ,
\end{align}
where the SM contributions are given by
\begin{align} 
 \left. \beta_{\lambda_H}^{(1)}\right\vert_{\mathrm{SM}}
 &=  12 \lambda^2_H +12 \lambda_H y^2_t  -12 y^4_t
    - \left(3 g_Y^2 +9 g_2^2\right) \lambda_H 
    +\frac{3}{4}g_{Y}^4 + \frac{3}{2}g_{Y}^{2} g_{2}^2 + \frac{9}{4}g_{2}^4 
    \ , \\
 \beta_{y_t}^{(1)}
 &=   y_t \left(
            \frac{9}{2} y^2_t 
            - \frac{17}{12} g_{Y}^{2} - \frac{9}{4} g_{2}^{2} -8 g_{3}^{2}
          \right) 
          \ .
					\label{eq:RGE:ytSM:oneloop}
\end{align}
\Eq{eq:RGE:lambdaH:oneloop} clearly shows that
the portal coupling $\lambda_{\phi H}$
has an effect of reducing the Higgs mass.


Figure~\ref{fig:Higgs:mass:pmoduli} shows our result.
We plot the $\suppress{R}=1$ case by the solid line,
which is to be compared with the $\suppress{R}=0$
shown by the dashed line.
%
%
Numerically,
if we compare these two cases
by the peak values of the calculated Higgs mass,
%in Fig.~\ref{fig:Higgs:mass:pmoduli},
then the reduction is of $1.17$\,\% ($1.57$\,\%)
for $\MS=1\nunits{TeV}$ ($2\nunits{TeV}$)
for unsuppressed $D$-term case $\suppress{D}=1$,
while it is reduced by $1.07$\,\% ($1.40$\,\%)
for completely suppressed $D$-term $\suppress{D}=0$.
We see that 
the inclusion of the pseudo-moduli
in the low-energy effective theory
does reduce the Higgs mass,
but such effect is only at most of a few percents.
As is expected,
such reduction becomes important
when the matching scale becomes large.


\begin{figure}[tbp]
 \begin{tabular}{lr}
  \begin{minipage}{0.45\hsize}
    \begin{center}
%#	\includegraphics[scale=0.8]{fig_mh-tanb_MS1_lamad03.eps}
	\includegraphics[scale=0.8]{fig_mh-tanb_MS2_CSSM.eps}
    \end{center}
  \end{minipage}
  \hspace{4mm}
  \begin{minipage}{0.45\hsize}
    \begin{center}
%#	\includegraphics[scale=0.8]{fig_mh-tanb_MS2_lamad03.eps}
	\includegraphics[scale=0.8]{fig_mh-tanb_MS1_CSSM.eps}
    \end{center}
  \end{minipage}
 \end{tabular}
\caption{
Upper bounds of the lightest Higgs mass as a function of $\tan\beta$. 
In each figure,
The matching to the SM with a light moduli is assumed
in the solid lines 
with the unsuppressed matching condition $\suppress{R}=1$,
while the dashed lines correspond
to the matching to the SM ($\suppress{R}=0$),
which are the same as the solid ones in 
the left panel of Fig.~\ref{fig:Higgs:mass:bound}.
The right (left) panel corresponds to the SUSY scale
$\MS=2\nunits{TeV}$ ($\MS=1\nunits{TeV}$), 
and as before,the blue and red lines correspond to
$\suppressionD{D}=1$ case and $\suppressionD{D}=0$ case,
respectively.
 }
%\label{fig:Higgs:mass:ad:03}
\label{fig:Higgs:mass:pmoduli}
\end{figure} 


%\clearpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> v2_changelog/sec4_width20160107b.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Constraints from Invisible Decays}
\label{sec:decay}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


In this section, 
we examine how the present model are constrained from 
invisible decays of the Higgs boson~\cite{Belanger:2013kya}
as well as the $Z$ boson. 
To calculate the mass and coupling of the pseudo-moduli,
we use as an input value at $\MS=1\nunits{TeV}$
of the singlet Yukawa coupling $\lambda =0.73$ 
that corresponds, at $\tan\beta=2$,
to the lightest Higgs mass $125\nunits{GeV}$. 
No radiative correction is taken into account in this section.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Mass and Interactions of Pseudo-Moduli}
\subsection{Mass  of Pseudo-Moduli}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


The present singlet extension of the minimal $R$-symmetric model 
contains a light scalar 
corresponding to a fluctuation along the ``pseudo-moduli'' direction.
As was described in \S{\ref{subsec:pmoduli}},
the pseudo-moduli $\phi$ can receive a mass $m^2_\phi$
from various sources
%, aside from $R$-symmetry breaking effects,
in the scalar potential \eq{eq:V}:
the $D$-term, adjoint Yukawa terms, as well as 
soft scalar masses of $R$-charged Higgses:
\begin{align}
m_\phi^2
\ =\ m^2_{\phi,F}+m^2_{\phi,D}+m^2_{\phi,A}+m^2_{\phi,\mathrm{soft}}
     \ .
\label{eq:moduli:mass}
\end{align}
For soft term,
we assume the form \eq{eq:V:soft:R},
%For definiteness, we assume that
%the pseudo-moduli receives from the soft terms of 
%the form \eq{eq:V:soft:R},
\begin{align}
%{}-\mathcal{L}_{\mathrm{soft}}
V_{\mathrm{soft},R}
\ =\ m^2_{R_0}\abs{R_0}^2
    +m^2_{R}\sum_{i=u,d}\abs{R_i}^2
     \ ,
\end{align}
where the soft mass $m_{R_0}$ of the singlet $R_0$
can be different from 
the common soft mass $m_{R}$ of the doublets $R_{u,d}$.
When all the $R$-charged Higgses 
have a universal soft mass $m^2_{R_0}=m^2_R(=m^2)$, 
the pseudo-moduli has a mass equal to $m^2_\phi=m^2$
and its mixing angles coincide with those of 
the pseudo-Goldstino states \eq{eq:moduli:state},
$U_{\phi I}=U_{\psi I}$ ($I=0,u,d$).


We are particularly interested in the limiting case,
$m^2_{R_0}\ll m^2_R$.
Figure~\ref{fig:moduli:mass} shows 
the mass eigenvalue of the pseudo-moduli state $\phi$,
in three particular cases,
$m^2_{R_0}=0$, $m^2_{R_0}=0.2\,m^2_R$ and $m^2_{R_0}=0.5\,m^2_R$.
From the figure, we see the following:
\begin{itemize}
\item
For a fixed value of $\mu$,
%The mass $m^2_\phi$ of the pseudo-moduli becomes large
the pseudo-moduli mass $m_\phi$ increases
by increasing the soft mass $m_R$ of $R_{u,d}$,
and approaches the singlet mass $m_{R_0}$
in the limit of large $m_R$.
In particular, if $m_{R_0}=0$,
it approaches 
the limiting value $\lambda v$, 
which is $126\nunits{GeV}$ for $\lambda=0.73$.
\item
%On the other hand, 
For a fixed value of $m_R$,
its mass $m_\phi$ decreases by increasing $\mu$.
This is because
the singlet component dominates 
the pseudo-moduli state
when $\mu$ is large compared to $\lambda v$. 
\end{itemize}
These behaviour can be understood from our estimate 
\eqs{eq:moduli:mass:mu:small}{eq:moduli:mass:mu:large}.


\begin{figure}[tbp]
 \begin{tabular}{cc}
  \begin{minipage}{0.45\hsize}
	\includegraphics[scale=0.8]{fig_moduli-mass_mu400.eps} 
  \end{minipage}
  \hspace{4mm}
  \begin{minipage}{0.45\hsize}
%\begin{center}
	\includegraphics[scale=0.8]{fig_moduli-mass_mr300.eps}
%\end{center}
  \end{minipage}
 \end{tabular}
\caption{
The pseudo-moduli mass $m_\phi$ as a function of
%the averaged Higgsino mass parameter $\mu$ (left) 
%and the common soft mass $m_R$ of $R$-charged doublets (right).
the averaged $\mu$ parameter (left) 
and the common doublet soft mass $m_R$ (right).
We take $\lambda =0.73$ and $\tan\beta=2$; %and 
$\mu=400{\rm GeV}$ in the left,
while $m_R=300{\rm GeV}$ in the right.
%Soft masses of doublet scalars  $R_d$, $R_u$ are commonly $m_R$. 
%
For the singlet soft mass $m_{R_0}$,
three cases $m_{R_0}/m_R=0$, $0.2$, and $0.5$ are shown
by blue dotted, red dashed and solid lines, respectively.
%
%$m_{R_0}=0$, $m_{R_0}=0.2m_R$, $m_{R_0}=0.5m_R$. 
	}
\label{fig:moduli:mass}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Interactions to the SM Higgs}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\mixing}[2]{\kappa_{{#1}{#2}}}
\renewcommand{\mixing}[2]{\delta_{{#1}}m_{#2}}

%%We denote the mass eigenstates in the $R$-charged sector
%%by $\phi_{J=1,2,3}$ where $\phi_1=\phi$ is the pseudo-moduli,
%%and define the mixing matrix $U_{IJ}$ by
%%\begin{align}
%%R_I^0
%%\ =\ \sum_{J=1,2,3}U_{IJ}\phi_J
%%   \ =\ U_{I\phi}\phi + \cdots
%%      \ ,
%%\end{align}


%defined by $V=g_{h\phi\phi}h\abs{\phi}^2$.
%In the notation of Ref.~\cite{Martin:1997ns},


Next we calculate the trilinear coupling $g_{h\phi\phi}$
of the lightest Higgs boson $h$ to the pseudo-moduli pair,
which also takes the form
\begin{align} 
g_{h\phi\phi}
\ =\ g_{h\phi\phi}^{(F)}+g_{h\phi\phi}^{(D)}+g_{h\phi\phi}^{(A)}
     \ .
\end{align} 
%corresponding to each term in the scalar potential \eq{eq:V}.
Let us take a close look at the first term
$g_{h\phi\phi}^{(F)}$ corresponding to the superpotential \eq{eq:W:Higgs}.
Substituting the usual expansion
%expression
%for the mixing angle $\alpha$ between $h$ and the heavier one $H'$,
\begin{align} 
	\begin{pmatrix}
		H_u\\
		H_d
	\end{pmatrix}
 &=
        v
	\begin{pmatrix}
		\sin\beta\\
		\cos\beta
	\end{pmatrix}
	+\frac{1}{\sqrt{2}} 
	\begin{pmatrix}
		\cos\alpha & \sin\alpha\\
		-\sin\alpha & \cos\alpha
	\end{pmatrix}
	\begin{pmatrix}
          h\\
          H'
	\end{pmatrix}
%        \ .
\nonumber
\end{align}
into the corresponding term $V_F$ in the scalar potential \eq{eq:V},
%From the superpotential \eq{eq:W:Higgs},
we obtain terms quadratic in the pseudo-moduli field $\phi$ as
\begin{align} 
% V_{H, \phi}
%{}-\mathcal{L}_\phi
V_{\phi,F}
 &=  m^2_{\phi,F}\abs{\phi}^2
     + g_{h\phi\phi}^{(F)} \abs{\phi}^2 h
     + \frac{1}{2}\,g_{hh\phi\phi}^{(F)} \abs{\phi}^2 h^2
     \ .
 \label{eq:Higgs-mod-int:F}
\end{align} 
Here the contributions to the mass and the trilinear coupling
are given by
\begin{align} 
m^2_{\phi,F}
 &=  \abs{\delta_u m_\phi}^2 + \abs{\delta_d m_\phi}^2
     \ ,
\\
%\end{align}
%and the trilinear coupling $g_{h\phi\phi}$ is given by
%\begin{align} 
% \kappa _u 
% &={}-\lambda U_{10} \sin\alpha
%      \ , \qquad
% \kappa _d
% \ =\ \lambda U_{10} \cos\alpha
%
 g_{h\phi\phi}^{(F)}
 &=  \frac{\lambda }{\sqrt{2}}
     \left[
       U^*_{0\phi}
       \Bigl(
         \delta_u m_{\phi\,}\sin\alpha - \delta_d m_{\phi\,}\cos\alpha
       \Bigr) + \mbox{c.c.}
     \right]
     \ ,
\end{align}
where
$U_{I\phi}=U^*_{\phi I}$ is 
the component of the lowest mass eigenstate $\phi$ 
in the fields $R_{I=0,u,d}$,
and we have defined
%the quantities $\mixing{i}{\phi_j}$ ($i=u,d$) are defined by
%%%\begin{align} 
%%% \mixing{u}{\phi_j}
%%% \equiv
%%%     \frac{\partial F_{H_u}}{\partial \phi_j}
%%% &=\,\mu_u U_{u\phi_j}-\lambda v_d U_{0\phi_j}
%%%%%     \ , \qquad
%%%%  ={}-\lambda v_d
%%%%      \left[
%%%%        U_{0\phi}-\frac{U_{u\phi}}{\tan\theta\cos\varphi}
%%%%      \right]
%%%      \ ,
%%%\nonumber\\
%%% \mixing{d}{\phi_j}
%%% \equiv
%%%     \frac{\partial F_{H_d}}{\partial \phi_j}
%%% &=\,\mu_d U_{d\phi_j}-\lambda v_u U_{0\phi_j}
%%%%     \ ,
%%%\end{align}
\begin{align} 
 \mixing{u}{\phi}
 \equiv
     \frac{\partial F_{H_u}}{\partial \phi}
 &=\,\mu_u U_{u\phi}-\lambda v_d U_{0\phi}
     \ , \qquad
\nonumber\\
 \mixing{d}{\phi}
 \equiv
     \frac{\partial F_{H_d}}{\partial \phi}
 &=\,\mu_d U_{d\phi}-\lambda v_u U_{0\phi}
      \ .
\end{align}
The quartic coupling $g_{hh\phi\phi}$ cam be found
in a similar manner;
we omit it here since it is irrelevant for later purpose.



%%%the quartic coupling $g_{hh\phi\phi}$ cam be found, 
%%%although it is irrelevant for later purpose, in a similar manner:
%%%if we denote the $i$-th mass eigenstate
%%%and its mass eigenvalue by $\phi_i$ and $m_i^2$,
%%%and define $\delta_u m_{\phi_i}=\partial F_{H_u}/\partial\phi_i$
%%%and similar for $\delta_d m_{\phi_i}$,
%%%\begin{align} 
%%%g_{hh\phi\phi}^{(F)}
%%% &=\  \lambda^2
%%%%      \left[ 
%%%	|U_{0\phi}|^2
%%%        -\frac{2|g_{h\phi\phi_2}|^2 }{m^2_2} 
%%%        - \frac{2|g_{h\phi\phi_3}|^2 }{m^2_3}
%%% %     \right] 
%%%      \ , 
%%%\\
%%%g_{h\phi\phi_i}
%%% &= \frac{\lambda}{\sqrt{2}}
%%%    \left[
%%%    U^*_{0\phi}
%%%   \Bigl(
%%%       \delta_u m_i \sin\alpha
%%%     - \delta_d m_i \cos\alpha
%%%   \Bigr)
%%% + U_{0\phi_i}
%%%   \Bigl(
%%%       \delta_u m_\phi \sin\alpha 
%%%     - \delta_d m_\phi \cos\alpha
%%%   \Bigr)^*
%%%   \right]
%%%   \ ,
%%%\nonumber \\
%%%m^2_i 
%%%  &= \abs{\delta_u m_{\phi_i}}^2 
%%%   + \abs{\delta_d m_{\phi_i}}^2
%%%   + \sum_{\alpha=0,u,d} m^2_{R\alpha }\abs{U_{\alpha\phi_i}}^2
%%%     \ .
%%%\end{align}
%%%where $\delta_{u,d} m_{\phi_i}$ are defined in a similar way as above.


Now, it is important to realize that
the pseudo-moduli mixing angles $U_{I\phi}$ ($I=0,u,d$)
coincide with pseudo-Goldstino angles \eq{eq:moduli:state},
$U_{I\phi}\rightarrow U_{I\psi}$,
if we neglect the terms in the scalar potential \eq{eq:V}
other than $V_F$;
The same is true 
if the soft masses are universal in the $R$-charged Higgs sector.
In these situations, we have 
%$U_{i\phi}\rightarrow U_{i\psi}$,
%so that
\begin{align} 
\delta_u m_{\phi}
\ ={}-\mu\sin\theta\cos\beta
      \left[
        \frac{U_{0\phi}}{\cos\theta}
        -\frac{U_{u\phi}}{\sin\theta\cos\varphi}
      \right]
 &\longrightarrow\ 0
      \ ,
\nonumber\\
\delta_d m_{\phi}
 \ ={}-\mu\sin\theta\sin\beta
      \left[
        \frac{U_{0\phi}}{\cos\theta}
        -\frac{U_{d\phi}}{\sin\theta\sin\varphi}
      \right]
 & \longrightarrow\ 0
  \ ,
\end{align}
which reflects the fact that
the pseudo-moduli $\phi$ does not get a mass from the Higgs VEV's.
It implies that %the pseudo-moduli 
$\phi$ decouples from the Higgs boson
in this limit.
In other words,
the trilinear interaction of a lightest Higgs and two pseudo-moduli
arises from a deviation of the pseudo-moduli eigenstate
from the would-be flat direction,
caused by the other terms in the scalar potential \eq{eq:V}.


The $D$-term contribution to the trilinear coupling 
is\,\footnote{
This contribution can take both signs,
as in the case of $D$-contributions to soft scalar masses.
}
\begin{align} 
% V_{h\phi \phi,D}
 g_{h\phi\phi}^{(D)}
\ ={}-\suppressionD{D\,}\frac{g_Z^2 v}{2\sqrt{2}}\,
      \sin\left(\alpha+\beta\right)
      \Big(
        \abs{U_{u\phi}}^2-\abs{U_{d\phi}}^2
      \Bigr)
      \ .
\label{eq:Higgs-mod-int:D}
\end{align}
This contribution is quite small, however,
in most of the parameter space: %by two reasons. 
%First, 
When $\mu$ or $m_R$ is larger than $\lambda v\sim 126\nunits{GeV}$,
the pseudo-moduli state is dominated by the singlet component,
so that the doublet components $U_{i\phi}$ ($i=u,d$) are small.
%Second,
Moreover, in the decoupling limit of the heavier Higgses, we have 
$\sin\left(\alpha+\beta\right)\rightarrow{}-\cos 2\beta
\left({}\sim 0.6\right)$,
giving another suppression
for a small $\tan\beta\left({}\sim 2\right)$.


%The contributions from the adjoint Yukawa terms \eq{eq:V:adjoint}
%may be important especially when
%the coupling $\lambdaad$ is large and
%$\lambdaad{}v$ is comparable to $\mu$ or $m_R$.


The adjoint Yukawa terms \eq{eq:V:adjoint}
also contribute, after the EW symmetry breaking,
to the mass matrix of $R$-charged Higgses
and the trilinear coupling to the Higgs boson
%--- [can be omitted from HERE]: 
%the mass matrix of $R$-charged Higgses,
%with abbreviations like $s_\alpha=\sin\alpha$,
%\begin{align} 
% V_{\textrm{ad},R}
% = 
% \begin{pmatrix}
%	R_u^{0\dagger} & R_d^{0\dagger}
% \end{pmatrix}\!\!
% \begin{pmatrix}
%     (\lambda ^{u2}_S + \lambda ^{u2}_T) s^2_\beta 
%   & (\lambda ^u_S \lambda ^d_S +\lambda ^u_T \lambda ^d_T)
%     s_\beta c_\beta 
%     \\
%     (\lambda ^u_S \lambda ^d_S +\lambda ^u_T \lambda ^d_T)
%     s_\beta c_\beta 
%   & (\lambda ^{d2}_S + \lambda ^{d2}_T)
%     c^2_\beta
% \end{pmatrix}
% \!v^2\!
% \begin{pmatrix}
%   R^0_u\\ R^0_d
% \end{pmatrix}
% \,, 
%\end{align}
%and [the END]---
%the trilinear coupling %interaction of Higgs and two moduli, 
\begin{align} 
 g_{h\phi\phi}^{(A)}
 = \sum_{a=S,T}
     \frac{v}{\sqrt{2}} 
     \left[ 
       \left(
           \lambda ^u_a U_{u\phi}\sin\beta 
         + \lambda ^d_a U_{d\phi}\cos\beta 
%           \lambda ^u_a U_{u\phi}s_\beta 
%         + \lambda ^d_a U_{d\phi}c_\beta 
       \right)
       \left(
           \lambda ^u_a U_{u\phi} \cos\alpha
         - \lambda ^d_a U_{d\phi}\sin\alpha
       \right)^*
     + \hbox{c.c.}
     \right] 
     \ .
\label{eq:Higgs-mod-int:ad}
\end{align}
This contribution is also small 
%for $\lambdaad{} v \ll \mu,\ m_R$,
%but can not be neglected if 
unless $\lambdaad{}v$ is comparable to $\mu$ or $m_R$.

%\def\thetamod{\theta_0}
%\def\phimod{\varphi_0}

%%%\blue{
%%%If we define the pseudo-moduli angles 
%%%$\thetamod$ and
%%%$\phimod$ in the $R$-charged scalar sector by 
%%%$U_{\phi0}=\cos\thetamod$,
%%%$U_{\phi u}=\cos\phimod\sin\thetamod$ and 
%%%$U_{\phi d}=\sin\phimod\sin\thetamod$,
%%%we then have for $\lambda_a^u=\lambda_a^d=\lambda_a$ case,
%%%\begin{align}
%%% g_{h\phi\phi}^{(A)}
%%% = \sum_{a=S,T}
%%%     \sqrt{2}\abs{\lambda_a}^2 v
%%%     \sin^2\thetamod
%%%     \sin\left(\phimod+\beta\right)
%%%     \cos\left(\phimod+\alpha\right)
%%%     \ .
%%%%\label{eq:Higgs-mod-int:ad}
%%%\end{align}
%%%}


Figure~\ref{fig:hmodmod-int} shows 
the trilinear coupling 
$g_{h\phi\phi}=g_{h\phi\phi}^{(F)}+g_{h\phi\phi}^{(D)}+g_{h\phi\phi}^{(A)}$ 
of the lightest Higgs and two pseudo-moduli.
%(over the Higgs VEV).
We see that
it is a increasing function of the soft mass $m_R$
as is expected;
it also decreases as $\mu$ becomes large,
since the singlet $R_0$ dominates in the eigenstate $\phi$.


\begin{figure}[tbp]
			\begin{tabular}{cc}
			\begin{minipage}{0.45\hsize}
	\includegraphics[scale=0.8]{fig_g-hphiphi_mu400.eps}
	\end{minipage}
\hspace{4mm}
			\begin{minipage}{0.45\hsize}
%\begin{center}
	\includegraphics[scale=0.8]{fig_g-hphiphi_mr300.eps}
%\end{center}
	\end{minipage}
\end{tabular}
\caption{
%The trilinear coupling of lightest Higgs and pseudo-moduli 
The trilinear coupling $g_{h\phi\phi}$
(divided by the Higgs  VEV) 
as a functions of $\mu$ and soft mass $m_R$ of $R_{u,d}$.
The parameters are the same 
as in the previous figure~\ref{fig:moduli:mass}.
%Input parameters are 
%$\lambda =0.73$, $\tan\beta=2$, 
%$\suppressionD{D}=0.5$ and $\tan\varphi=2.5$. 
%%Soft masses of doublet scalars  $R_u$, $R_d$ are commonly $m_R$. 
%Blue broken line, red broken line and black real line show 
%each singlet soft mass $m_{R_0}=0$, $m_{R_0}=0.2m_R$, $m_{R_0}=0.5m_R$. 
%The left figure is function $m_R$ at $\mu=400{\rm GeV}$ 
%and the right figure is function $\mu$ at $m_R=300{\rm GeV}$.  
	}
	\label{fig:hmodmod-int}
\end{figure}


%%The coupling $g_{hh\phi\phi}$ is shown in Fig.~\ref{fig:g-phi2h2},
%%although it is irrelevant here.
%%\begin{figure}[tbp]
%%  \begin{center}
%%		\includegraphics[scale=0.8]{fig_g-hhphiphi.eps}
%%  \end{center}
%%\caption{
%%The coupling $g_{hh\phi\phi}$
%%%of two lightest Higgs and two pseudo-moduli 
%%as a functions of the common soft mass $m_R$.
%%%of R-charged Higgs scalars. 
%%Input parameters are 
%%$\lambda =0.75$, $\tan\beta=2$, 
%%$\suppressionD{D}=0$, $\mu=1000{\rm GeV}$ and $\tan\varphi=2.5$. 
%%%Soft masses of doublet scalars  $R_u$, $R_d$ are commonly $m_R$. 
%%}
%%\label{fig:g-phi2h2}
%%\end{figure}


In passing, we note that
In the decoupling limit of heavier Higgses,
where $\alpha\rightarrow\beta-\pi/2$,
Eqs.~(\ref{eq:Higgs-mod-int:F}), 
\eqs{eq:Higgs-mod-int:D}{eq:Higgs-mod-int:ad}
are slightly simplified as
\begin{align} 
 g_{h\phi\phi}^{(F)}
 &\longrightarrow{}
      \sqrt{2} \lambda^2 v |U_{0\phi}|^2 
     -\frac{\lambda}{\sqrt{2}}
      \left[ U_{0\phi}^*
        \Bigl(
          \mu_u U_{u\phi}\cos\beta +\mu_d U_{d\phi} \sin\beta 
        \Bigr)
        +\hbox{c.c}
      \right]
      \ ,
\\
 g_{h\phi\phi}^{(D)}
 &\longrightarrow{}
      \sqrt{2}\,\frac{g^2_Z}{4}\,v\,\cos2\beta 
      \Bigl(
        \abs{U_{u\phi}}^2-\abs{U_{d\phi}}^2
      \Bigr)
      \ ,
\\
 g_{h\phi\phi}^{(A)}
 &\longrightarrow{}
      \sqrt{2}
      \sum_{a=S,T}
      v
      \left|
        \lambda ^u_a U_{u\phi} \sin\beta 
        + \lambda ^d_a U_{d\phi} \cos\beta 
      \right|^2
      \ .
\end{align}


%we have $\alpha\rightarrow\beta-\pi/2$.
%Accordingly,



%\blue{
%%Note:
%\begin{itemize}
%\item
%in \S{\ref{sec:triviality}},
%we take the decoupling limit $m_A\rightarrow\infty$
%so that $\tan\alpha={}-\cot\beta$.
%\item
%in \S{\ref{sec:decay}},
%we take $m_A=1\nunits{TeV}$ and $\tan\beta=2$
%so that $\tan\alpha={}-0.46$.
%In this case,
%the deviations in the up (down)-type Yukuwa couplings from the SM ones
%are estimated to be about $+0.2\%$ ($-0.8\%$).
%\end{itemize}
%}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Bounds from Invisible Decays}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Having calculated the mass and the interaction
of the pseudo-moduli,
we now examine the constraints from the invisible decays.


First let us briefly discuss the constraint 
from invisible decay of the Z boson.
%In the present model, 
Since we are supposing that explicit $R$ symmetry breaking
%is very small as was discussed in Ref.~\cite{Morita:2012kh},
is very small \cite{Morita:2012kh},
we treat the pseudo-Goldstino $\psi$ as massless
in the following.
%so that $Z$ can decay to $\psi\psi^\dagger$ pair.
%Consequently we should discuss the devay of $Z\rightarrow \psi\psi$.


The $Z$ coupling of the pseudo-Goldstinos 
comes from the neutral current
%can be read off from the neutral current of the doublet components
%$\wt{R}_{u,d}^0$,
\begin{align} 
  \left.J_{Z}^\mu\right\vert_{\wt{R}}
\ =\ 
        \frac{g_Z}{2}\left[
           \wt{R}^{0\dagger} _d \wb{\sigma}^\mu \wt{R}_d^0
          -\wt{R}^{0\dagger}_u \wb{\sigma}^\mu \wt{R}_u^0
        \right]
\ ={}- \frac{g_Z}{2}\,
        \psi^\dagger \wb{\sigma}^\mu\psi\,
        \sin^2\theta \cos{2\varphi}
        +\cdots
        \ , 
\label{eq:Zpsipsi:int}
\end{align}
with the mixing angles $\theta$ and $\varphi$ 
defined by \Eq{eq:angle:def}.
The decay width of $Z\to \psi\psi^\dagger$ is then
\begin{align} 
 \Gamma_{Z\to \psi\psi}
 \ =\ \frac{g^2_Z m_Z}{96 \pi}
       \left(\sin^2\theta \cos{2\varphi}\right)^2 
%       \left(\sin^2\theta \cos\left(2\varphi\right)\right)^2 
       \ .
\label{eq:Zpsipsi:width}
\end{align}
Requiring that this is less than 
the error of the measured value~\cite{Agashe:2014kda} of the total width 
$ \Gamma _Z\ =\ 2.4952\pm0.0023\nunits{GeV}$,
%\begin{align} 
% \Gamma _Z\ =\ 2.4952\pm0.0023\nunits{GeV}
% \ ,
%%\label{eq:width:Z}
%\end{align}
we obtain the bound
\begin{align} 
% \abs{\sin^2\theta \cos{2\varphi}}\ \leq\ 0.117
  \abs{\sin^2\theta \cos{2\varphi}}\ \leq\ 0.0988
  \ .
\end{align}
%which is depicted in Fig.~\ref{fig:zinv2}.


\begin{figure}[btp]
  \begin{center}
		\includegraphics[scale=0.8]{fig_Z-inv.eps}
  \end{center}
\caption{
The constraint from invisible decay of the Z boson.
The gray region is excluded. 
The vertical axis is the mixing angle $\cot\theta=\mu/\lambda{}v$ 
between the singlet/doublet components of 
$R$-charged Higgsinos, $\wt{R}_0$ and $\wt{R}_{u,d}^0$,
while the horizontal axis is the angle $\tan\varphi$ 
within $\wt{R}_{u,d}^0$.
         }
\label{fig:zinv2}
\end{figure}


The bound is depicted in Fig.~\ref{fig:zinv2}.
Recall that 
$\tan\theta=\lambda{}v/\mu$ is the mixing angle 
between the singlet and doublet components of $R$-charged Higgsinos,
$\wt{R}_0$ and $\wt{R}_{u,d}^0$.
For a generic value of $\tan\varphi$, 
which is the angle between $\wt{R}_u$ and $\wt{R}_d$,
a smaller value of $\mu$ implies that
the pseudo-Goldstino $\psi$ has a larger doublet component
and thus more strongly couples to the $Z$ boson.
We see that 
the constraint can easily be satisfied
if the averaged Higgsino mass parameter $\mu$ 
is larger than $\lambda v$:
For $\lambda=0.73$, we get a lower bound $\mu \gtrsim 285\nunits{GeV}$.
% $\mu \gtrsim 220\nunits{GeV}$. 
Then the chargino mass bounds from direct searches are also satisfied.
We add that
%the constraint is weak 
the pseudo-Goldstino becomes almost decoupled from the $Z$ boson
for $\tan\varphi=\left(\mu_u/\mu_d\right)\tan\beta \approx 1$,
or equivalently,
for $\tan\beta\approx\mu_d/\mu_u$
as is the case if the soft masses of $H_{u,d}$ are small.


%We note that
The $Z$ boson can decay also into
a pair of the pseudo-moduli $\phi$
if the latter is lighter than $m_Z/2$.
This corresponds to
$m_R\lsim 150\nunits{GeV}$ for $\mu=400\nunits{GeV}$ and
$\mu\gsim 700\nunits{GeV}$ for $m_R=300\nunits{GeV}$,
as is seen from Fig.~\ref{fig:moduli:mass}. 
The partial decay width for $Z\to \phi\phi^\dagger$
\begin{align} 
 \Gamma_{Z\to \phi\phi} 
\  =\ \frac{g^2_Z m_Z}{96 \pi}
       \Bigl(\abs{U_{u\phi}}^2-\abs{U_{d\phi}}^2\Bigr)^2 
       \left(1-\frac{4m^2_\phi}{m^2_Z}\right)^{3/2} 
\end{align}
%This contribution 
approaches that of $Z\to\psi\psi^\dagger$ %, \Eq{eq:Zpsipsi:width},
in the limit of small $m_R$,
but becomes negligible if 
the soft mass $m_R$ is as large as $100\nunits{GeV}$.


%Figure~\ref{fig:Higgs:inv:Zadd} shows 
%additional contribution of Z to two pseudo-moduli 
%by  Fig.~\ref{fig:Higgs:inv:decay} and \ref{fig:higgs:inv:adjoint}. 


%\paragraph{Higgs width}


Next we discuss the invisible width of the Higgs boson.
If the pseudo-moduli $\phi$ is lighter than $m_h/2$,
the Higgs boson can decay into a pair of $\phi$.
%which contributes to the invisible width of the Higgs boson.
%The decay width for $h\to\phi\phi^\dagger$ is given by
The decay width for $h\to\phi\phi^\dagger$ is given 
in terms of the trilinear coupling $g_{h\phi\phi}$ 
and the pseudo-moduli mass $m_\phi$
by\,\footnote{
The decay $h\to\psi\wb{\psi}$ is negligible
%since $\psi$ does not get a mass from the Higgs VEV.
since 
it is proportional to $m_\psi$
(modulo a loop-suppressed contribution)
and $m_\psi$ vanishes in the $R$-symmetric limit.
}
\begin{align} 
 \Gamma _{h\to\phi\phi}
\ =\ 
%     \frac{g^2_{h\phi\phi}}{32\pi m_h}\,
     \frac{g^2_{h\phi\phi}}{16\pi m_h}\,
     \sqrt{1-\frac{4m^2_\phi}{m^2_h}}
     \ .
\end{align}
%where $g_{h\phi\phi}$ is the coupling of the Higgs and two moduli
%and $m_\phi$ is the pseudo-moduli mass. 
%
We require that 
%the invisible Higgs decay width 
this width should be smaller 
than the partial width of $h \to b\wb{b}$ in the SM,
\begin{align} 
 \Gamma_{h\rightarrow\phi\phi}
\ <\ \Gamma_{h\rightarrow bb} ^{\mathrm{SM}}
\ \approx\ 2.34\times 10^{-3}\nunits{GeV}
        \ ,
\end{align}
where $\Gamma^{\mathrm{SM}} _h=4.07\times 10^{-3} \nunits{GeV}$
and $\mathrm{Br}\!\left({h \to b\wb{b}}\right)=57.7 \% $
are the SM predictions \cite{Agashe:2014kda}.


%For the total decay width and branching ratio of the Higgs boson,
%\begin{align} 
% \Gamma _h
% &= 4.07\times 10^{-3} \nunits{GeV}
% \ , 
%\label{eq:width:H}
%\end{align}
%and branching ratio of $h \to bb$ is $57.7 \% $.  


Figure~\ref{fig:Higgs:inv:decay} shows
the resulting bound on parameters $\mu$ and $m_R$. 
%by invisible decay of the lightest Higgs boson 
The left panel corresponds to the $m_{R_0}=0$ case,
in which an excluded region appears
once the pseudo-moduli mass $m_\phi$ (shown by the dashed lines)
is smaller than $m_h/2$.
Remarkably and unlike a generic expectation,
the constraint becomes weak and disappears
as the pseudo-moduli becomes lighter and lighter.
We also see from the right panel that
the constraint is milder 
for the singlet soft mass $m_{R_0}\neq0$.
Actually it disappears 
if the $\mu$ parameter is as large as $1\nunits{TeV}$.


In the figures,
we also show the contours of future reaches
for the branching ratio of invisible Higgs decays,
for which we quote 
$9\%$ for the LHC with $3000\nunits{fb}^{-1}$
at $\sqrt{s}=14\nunits{TeV}$ \cite{Okawa:2013hda},
and $0.4\%$ for the ILC with $1150\nunits{fb}^{-1}$ 
at $\sqrt{s}=250\nunits{GeV}$ \cite{Asner:2013psa}.
We need other constraints, 
for instance from direct searches for charginos,
to cover the whole parameter space.


The reason for this behaviour is that
the lighter $\phi$ implies the smaller $g_{h\phi\phi}$ coupling.
As a comparison,
we also show in Fig.~\ref{fig:higgs:inv:adjoint}
the corresponding bound in the case of $\lambdaad=0.4$. 
In this case, the would-be pseudo-moduli direction 
is deformed by adjoint couplings
and consequently the constraints from the invisible decay
become slightly tight.
We see that a larger parameter region can be probed in a future,
especially when the soft mass $m_R$ is small.


\begin{figure}[tbp]
 \begin{tabular}{cc}
  \begin{minipage}{0.45\hsize}
	\includegraphics[scale=0.5]{fig_Higgs-inv_mr0-0mr_light.eps}
  \end{minipage}
  \hspace{4mm}
  \begin{minipage}{0.45\hsize}
	\includegraphics[scale=0.5]{fig_Higgs-inv_mr0-02mr_light.eps}
%\end{center}
  \end{minipage}
 \end{tabular}
\caption{
The constraints from invisible $Z$ and Higgs decays
in $\left(\mu,m_R\right)$ plane.
%The horizontal (vertical) axis is $\mu$ ($m_R$), respectively.
The input parameters are $\tan\beta=2$, $\tan\varphi=2.5$,
$\suppressionD{D}=0.5$ and $\lambda =0.73$ at $\MS=1\nunits{TeV}$.
%The upper (lower) figures correspond to $\lambda =0.75$ ($0.50$).
In the left panel, we take $m_{R_0}=0$ 
while $m_{R_0}=0.2\, m_{R}$ in the right.
The purple and Gray regions are excluded 
by invisible decay of the $Z$ and Higgs, respectively.
The black solid contour corresponds to $m_\phi=m_h/2$,
while the dashed contours correspond to
$m_\phi=\{30, 50, 80, 100\}\nunits{GeV}$, respectively, from the bottom.
Future reaches of 
the LHC ($\mathrm{Br}=0.09$) and ILC ($\mathrm{Br}=0.004$)
are also shown by the blue and red lines, respectively.
	}
\label{fig:Higgs:inv:decay} 
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[tbp]
 \begin{tabular}{cc}
 \begin{minipage}{0.45\hsize}
	\includegraphics[scale=0.5]{fig_Higgs-inv_lamad04_mr0-0mr_light.eps}
  \end{minipage}
  \hspace{4mm}
  \begin{minipage}{0.45\hsize}
	\includegraphics[scale=0.5]{fig_Higgs-inv_lamad04_mr0-02mr_light.eps}
  \end{minipage} 
\end{tabular}
 \caption{
The same as in Fig.~\ref{fig:Higgs:inv:decay},
but with the adjoint Yukawa couplings
$\lambdaad=0.4$.
%$\lambda^u_S=\lambda^d_S=\lambda^u_T=\lambda^d_T=0.4$.
%
	}
\label{fig:higgs:inv:adjoint} 
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\paragraph{Note on input and output parameters}


As a reference,
we show two sets of sample parameters
in Table~\ref{tab:input:output}.
We take the averaged Higgsino mass $\mu$ equal to $\MS$,
while the ratio is given by $\mu_u/\mu_d=\tan\varphi/\tan\beta=1.25$.
The values of $\tan\alpha$ correspond to our input that 
the pseudo-scalar Higgs mass is equal to $\MS$.
The value of $\tan\alpha$ follows from taking 
the pseudo-scalar Higgs mass equal to $\MS$,
and implies $0.2\,\%$ enhancement ($0.8\,\%$ reduction)
of the up-type (down-type) Yukawa interactions.
The adjoint scalar masses according to 
$m^2_{\sigma_a}/8=8m^2_{\pi_a}=m^2_{D_a}$ for each $a=1,2,3$
leads to the $D$-term suppression $\suppress{D}=1/2$.


\input table3_inputs20151207a.tex


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> v2_changelog/sec5_conclusion20160107a.tex <==
%\clearpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Summary and Discussion}
\label{sec:summary}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


We have studied a singlet extension of
the minimal $R$-symmetric SUSY SM with Dirac gauginos
that is consistent with gauge coupling unification.
Specifically we have calculated the mass of the SM-like Higgs boson
and found that 
its observed value of $125\nunits{GeV}$ can well be reproduced
in a small $\tan\beta$ region,
by the nMSSM-like, singlet Yukawa coupling $\lambda$
within perturbativity up to the unification scale
$10^{16}$--$10^{17}\nunits{GeV}$.
This is true even when the SUSY scale is as low as $1\nunits{TeV}$
and, remarkably, even without the standard $D$-term contribution
to the quartic Higgs potential.
The latter is important because
the $D$-term potential is known to be suppressed
in theories of Dirac gauginos and supersoft SUSY breaking.


The unification is preserved in a minimal way
by adding two vector-like pairs of singlet ``leptons''.
Adding more extra matters makes the gauge couplings stronger at UV
and thus relaxes the triviality bound.
We also examined the precision of unification by using two-loop RGE's.
Although we have not taken into account
the full variety of SUSY particle threshold,
we found that
a heavier Dirac gluino and/or wino makes the unification precise.
We note that
the mass threshold of a Dirac gaugino combined with
its scalar partners, $\sigma$ and $\pi$,
can conveniently be represented at one-loop by a single mass scale 
$M_D=\left(m_D^8 m_\sigma m_\pi\right)^{1/10}$.


The allowed parameter space is rather limited
in a small $\tan\beta$ region
especially when $SU(2)\times U(1)$ $D$-terms are suppressed
by adjoint scalar contributions.
Recent dedicated calculations 
\cite{Goodsell:2014pla,Diessner:2015yna}
show, however, that a part of two-loop contributions
gives substantial improvement of the Higgs mass
in the singlet extensions of the MSSM;
This is also the case in models that contains Dirac gluino.
It would imply that
our calculation based on RG method
may underestimate the upper bound of the Higgs mass
and that there are broader parameter region
that is consistent with the triviality bound.


A characteristic feature of the present $R$-symmetric model
is the existence of light scalar and fermion modes, 
pseudo-moduli $\phi$ and pseudo-Goldstino $\psi$,
whose properties are restricted by the approximate $U(1)_R$ symmetry.
Although the mixing between the pseudo-moduli and the SM Higgs
is negligible,
it does affect the RG evolution of the SM Higgs quartic coupling
below the SUSY scale.
We have examined this effect 
by constructing
%as the low-energy effective theory below the SUSY scale
the SM coupled with the pseudo-moduli
and found that
the Higgs mass is reduced by a few \%,
but there exists a parameter region
consistent with $125\nunits{GeV}$ Higgs,
again even without $D$-term.



As we discussed,
the constraints from invisible decays of the $Z$ and Higgs bosons
are weak if the singlet component dominates the lightest mass eigenstates.
The constraint from the $Z$ decay can easily be satisfied
since the present model contains the Higgsino mass parameters.
On the other hand,
the invisible Higgs decay generically
gives a tight constraint, 
as was originally expected.
We have found, however, that
there are interesting regions of parameter space
that the Higgs invisible width is within the current bound
and within the proposed reaches of the future experiments:
This occurs especially when 
the Higgsino mass parameters are much larger
than $\lambda v$ of order of $100\nunits{GeV}$.

There remain many issues to be discussed.
First, improved calculations 
including full SUSY spectrum 
and higher loop corrections are desired.
The invisible Higgs decay 
in the $R$-symmetric setup
should be studied in more general manner;
we have explored a limited region of parameter space.
For instance, if the singlet soft mass is larger than the doublet ones,
the lightest mass eigenstate $\phi$
deviates from the original pseudo-moduli direction.
This implies that 
the $\phi$ becomes heavier but has a larger coupling to the Higgs.
Loop corrections may also be important
since the suppression of the pseudo-moduli coupling
to the Higgs boson depends on a specific structure
of the potential.
Detailed studies about the adjoint Yukawa couplings
and their upper bound should be done.
On a theoretical side,
it is also important to justify the assumptions
about the origin or the absence of superpotential terms
that we mentioned in \S\ref{sec:setup}.
Finally we should remark that
cosmology of the singlet extended $R$-symmetric model
is still challenging and deserves further study.


%\clearpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> v2_changelog/sec6_reference20160107a.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{thebibliography}{99}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% Intro 
%%%%% For U(1)_R


\bibitem{Giudice:2011cg}
  G.~F.~Giudice and A.~Strumia,
  %``Probing High-Scale and Split Supersymmetry with Higgs Mass Measurements,''
  Nucl.\ Phys.\ B {\bf 858} (2012) 63
%  doi:10.1016/j.nuclphysb.2012.01.001
  [arXiv:1108.6077 [hep-ph]].

\bibitem{Hall:1990hq}
  L.~J.~Hall and L.~Randall,
  %``U(1)-R symmetric supersymmetry,''
  Nucl.\ Phys.\ B {\bf 352} (1991) 289.

\bibitem{Randall:1992cq}
  L.~Randall and N.~Rius,
  %``The Minimal U(1)-R symmetric model revisited,''
  Phys.\ Lett.\ B {\bf 286} (1992) 299.


\bibitem{Fox:2002bu}
  P.~J.~Fox, A.~E.~Nelson and N.~Weiner,
  %``Dirac gaugino masses and supersoft supersymmetry breaking,''
  JHEP {\bf 0208} (2002) 035
  [hep-ph/0206096].


 %%%%% supersafe 
\bibitem{Heikinheimo:2011fk}
  M.~Heikinheimo, M.~Kellerstein and V.~Sanz,
  %``How Many Supersymmetries?,''
  JHEP {\bf 1204} (2012) 043
  [arXiv:1111.4322 [hep-ph]].

\bibitem{Kribs:2012gx}
  G.~D.~Kribs and A.~Martin,
  %``Supersoft Supersymmetry is Super-Safe,''
  Phys.\ Rev.\ D {\bf 85} (2012) 115014
  [arXiv:1203.4821 [hep-ph]].

%%%%% min. R-symmetric model: def, flavor safe

\bibitem{Kribs:2007ac}
  G.~D.~Kribs, E.~Poppitz and N.~Weiner,
  %``Flavor in supersymmetry with an extended R-symmetry,''
  Phys.\ Rev.\ D {\bf 78} (2008) 055010
  [arXiv:0712.2039 [hep-ph]].

%%% CP in Dirac gaugino

\bibitem{Hisano:2006mv}
  J.~Hisano, M.~Nagai, T.~Naganawa and M.~Senami,
  %``Electric Dipole Moments in PseudoDirac Gauginos,''
  Phys.\ Lett.\ B {\bf 644} (2007) 256
  [hep-ph/0610383].


%%% FCNC in min. R

\bibitem{Fok:2010vk}
  R.~Fok and G.~D.~Kribs,
  %``\mu to e in R-symmetric Supersymmetry,''
  Phys.\ Rev.\ D {\bf 82} (2010) 035010
  [arXiv:1004.0556 [hep-ph]].

\bibitem{Dudas:2013gga}
  E.~Dudas, M.~Goodsell, L.~Heurtier and P.~Tziveloglou,
  %``Flavour models with Dirac and fake gluinos,''
  Nucl.\ Phys.\ B {\bf 884} (2014) 632
  [arXiv:1312.2011 [hep-ph]].

%%%%% pheno. of min. R-symmetric Higgs sector

\bibitem{Choi:2010an}
  S.~Y.~Choi, D.~Choudhury, A.~Freitas, J.~Kalinowski and P.~M.~Zerwas,
  %``The Extended Higgs System in $R$-symmetric Supersymmetry Theories,''
  Phys.\ Lett.\ B {\bf 697} (2011) 215; 
%erratum
   [Phys.\ Lett.\ B {\bf 698} (2011) 457]
  [arXiv:1012.2688 [hep-ph]].

%%% CP and EWBG in Dirac gaugino

\bibitem{Kumar:2011np}
  P.~Kumar and E.~Ponton,
  %``Electroweak Baryogenesis and Dark Matter with an approximate R-symmetry,''
  JHEP {\bf 1111} (2011) 037
  [arXiv:1107.1719 [hep-ph]].

%%% CP and EWBG in MRSSM

\bibitem{Fok:2012fb}
  R.~Fok, G.~D.~Kribs, A.~Martin and Y.~Tsai,
  %``Electroweak Baryogenesis in R-symmetric Supersymmetry,''
  Phys.\ Rev.\ D {\bf 87} (2013) 5,  055018
  [arXiv:1208.2784 [hep-ph]].



%%%%% other models with R-symmetry

\bibitem{Frugiuele:2012pe}
  C.~Frugiuele, T.~Gregoire, P.~Kumar and E.~Ponton,
  %``'L=R' - $U(1)_R$ as the Origin of Leptonic 'RPV',''
  JHEP {\bf 1303} (2013) 156
  [arXiv:1210.0541 [hep-ph]].


\bibitem{Morita:2012kh}
  Y.~Morita, H.~Nakano and T.~Shimomura,
  %``Neutrino Mass and Proton Decay in a ${U(1)}_R$ Symmetric Model,''
  PTEP {\bf 2013} (2013) 053B02
  [arXiv:1212.4304 [hep-ph]].


\bibitem{Chakraborty:2013gea} 
  S.~Chakraborty and S.~Roy,
  %``Higgs boson mass, neutrino masses and mixing and keV dark matter 
  %in an $U(1)_R-$ lepton number model,''
  JHEP {\bf 1401}, 101 (2014)
  [arXiv:1309.6538 [hep-ph]].


%%%%% non R model: [min.DG SUSY SM]

\bibitem{Benakli:2014cia}
  K.~Benakli, M.~Goodsell, F.~Staub and W.~Porod,
  %``Constrained minimal Dirac gaugino supersymmetric standard model,''
  Phys.\ Rev.\ D {\bf 90} (2014) 4,  045017
  [arXiv:1403.5122 [hep-ph]].


%%%%% min. R-symmetric model: Higgs mass

\bibitem{Bertuzzo:2014bwa}
  E.~Bertuzzo, C.~Frugiuele, T.~Gregoire and E.~Ponton,
  %``Dirac gauginos, R symmetry and the 125 GeV Higgs,''
  JHEP {\bf 1504} (2015) 089
  [arXiv:1402.5432 [hep-ph]].

\bibitem{Diessner:2014ksa}
	P.~Diessner, J.~Kalinowski, W.~Kotlarski and D.~Stoeckinger,
  %``Higgs boson mass and electroweak observables in the MRSSM,''
  JHEP {\bf 1412} (2014) 124
  [arXiv:1410.4791 [hep-ph]].

\bibitem{Diessner:2015yna}
  P.~Diessner, J.~Kalinowski, W.~Kotlarski and D.~Stockinger,
  %``Two-loop correction to the Higgs boson mass in the MRSSM,''
  Adv.\ High Energy Phys.\  {\bf 2015} (2015) 760729
  [arXiv:1504.05386 [hep-ph]].

\bibitem{Nelson:2002ca}
  A.~E.~Nelson, N.~Rius, V.~Sanz and M.~Unsal,
  %``The Minimal supersymmetric model without a mu term,''
  JHEP {\bf 0208} (2002) 039
  [hep-ph/0206102].


%%%%% multople SUSY breaking:


%%%%% INS superpotential

\bibitem{Izawa:2011hi}
  K.~I.~Izawa, Y.~Nakai and T.~Shimomura,
  %``Higgs Portal to Visible Supersymmetry Breaking,''
  JHEP {\bf 1103} (2011) 007
  [arXiv:1101.4633 [hep-ph]].

\bibitem{Bertolini:2011tw}
  D.~Bertolini, K.~Rehermann and J.~Thaler,
  %``Visible Supersymmetry Breaking and an Invisible Higgs,''
  JHEP {\bf 1204} (2012) 130
  [arXiv:1111.0628 [hep-ph]].



%%%%% DG ext. MSSM

%\bibitem{Belanger:2009wf}
%  G.~Belanger, K.~Benakli, M.~Goodsell, C.~Moura and A.~Pukhov,
%  %``Dark Matter with Dirac and Majorana Gaugino Masses,''
%  JCAP {\bf 0908} (2009) 027
%  [arXiv:0905.1043 [hep-ph]].


%%%%% review on NMSSM
\bibitem{Ellwanger:2009dp}
  U.~Ellwanger, C.~Hugonie and A.~M.~Teixeira,
  %``The Next-to-Minimal Supersymmetric Standard Model,''
  Phys.\ Rept.\  {\bf 496} (2010) 1
  [arXiv:0910.1785 [hep-ph]].

%%% singlet-doublet mixing at large tan beta
\bibitem{Badziak:2013bda}
  M.~Badziak, M.~Olechowski and S.~Pokorski,
  %``New Regions in the NMSSM with a 125 GeV Higgs,''
  JHEP {\bf 1306} (2013) 043
  [arXiv:1304.5437 [hep-ph]].

%%%%% NMSSM higgs mass
\bibitem{Ellwanger:2012ke}
  U.~Ellwanger and C.~Hugonie,
  %``Higgs bosons near 125 GeV in the NMSSM with constraints at the GUT scale,''
  Adv.\ High Energy Phys.\  {\bf 2012} (2012) 625389
  [arXiv:1203.5048 [hep-ph]].

\bibitem{Kobayashi:2012ee}
  T.~Kobayashi, H.~Makino, K.~i.~Okumura, T.~Shimomura and T.~Takahashi,
  %``TeV scale mirage mediation in NMSSM,''
  JHEP {\bf 1301} (2013) 081
  [arXiv:1204.3561 [hep-ph]].

\bibitem{Goodsell:2014pla}
  M.~D.~Goodsell, K.~Nickel and F.~Staub,
  %``Two-loop corrections to the Higgs masses in the NMSSM,''
  Phys.\ Rev.\ D {\bf 91} (2015) 035021
  [arXiv:1411.4665 [hep-ph]].


%%%%% nMSSM: Z_5 R

\bibitem{Panagiotakopoulos:1999ah}
  C.~Panagiotakopoulos and K.~Tamvakis,
  %``New minimal extension of MSSM,''
  Phys.\ Lett.\ B {\bf 469} (1999) 145
%  doi:10.1016/S0370-2693(99)01247-2
  [hep-ph/9908351].

\bibitem{Panagiotakopoulos:2000wp}
  C.~Panagiotakopoulos and A.~Pilaftsis,
  %``Higgs scalars in the minimal nonminimal supersymmetric standard model,''
  Phys.\ Rev.\ D {\bf 63} (2001) 055003
  [hep-ph/0008268].


%%%%% nMSSM at TeV scale:
\bibitem{Ishikawa:2014owa}
  K.~Ishikawa, T.~Kitahara and M.~Takimoto,
  %``Singlino Resonant Dark Matter and 125 GeV Higgs Boson 
  %in High-Scale Supersymmetry,''
  Phys.\ Rev.\ Lett.\  {\bf 113} (2014) 13,  131801
  [arXiv:1405.7371 [hep-ph]].

%\bibitem{Kitahara:2015wia}
%  T.~Kitahara,
%  %``Aspects of High-Scale Supersymmetry in a Singlet-Extended Model,''
%  arXiv:1508.04810 [hep-ph].

%%%%% PQ-NMSSM:
\bibitem{Jeong:2011jk}
  K.~S.~Jeong, Y.~Shoji and M.~Yamaguchi,
  %``Peccei-Quinn invariant extension of the NMSSM,''
  JHEP {\bf 1204} (2012) 022
  [arXiv:1112.1014 [hep-ph]].

\bibitem{Jeong:2012ma}
  K.~S.~Jeong, Y.~Shoji and M.~Yamaguchi,
  %``Singlet-Doublet Higgs Mixing and Its Implications 
  %on the Higgs mass in the PQ-NMSSM,''
  JHEP {\bf 1209} (2012) 007
  [arXiv:1205.2486 [hep-ph]].

% light higgsino in PQ-NMSSM
\bibitem{Choi:2013lda}
  K.~Choi, S.~H.~Im, K.~S.~Jeong and M.~S.~Seo,
  %``Higgs phenomenology in the Peccei-Quinn invariant NMSSM,''
  JHEP {\bf 1401} (2014) 072
  [arXiv:1308.4447 [hep-ph]].


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% setup


\bibitem{Kojima:2011ad} 
  K.~Kojima, K.~Takenaga and T.~Yamashita,
  %``Grand Gauge-Higgs Unification,''
  Phys.\ Rev.\ D {\bf 84}, 051701 (2011)
  [arXiv:1103.1234 [hep-ph]].


%%%%% supersoft operator

\bibitem{Polchinski:1982an}
  J.~Polchinski and L.~Susskind,
  %``Breaking of Supersymmetry at Intermediate-Energy,''
  Phys.\ Rev.\ D {\bf 26} (1982) 3661.

%%%%% D-term breaking

\bibitem{Itoyama:2011zi}
  H.~Itoyama and N.~Maru,
  %``D-term Dynamical Supersymmetry Breaking Generating 
  %Split N=2 Gaugino Masses of Mixed Majorana-Dirac Type,''
  Int.\ J.\ Mod.\ Phys.\ A {\bf 27} (2012) 1250159
  [arXiv:1109.2276 [hep-ph]].

\bibitem{Itoyama:2012fk}
  H.~Itoyama and N.~Maru,
  %``D-term Dynamical SUSY Breaking,''
  Int.\ J.\ Mod.\ Phys.\ Conf.\ Ser.\  {\bf 21} (2013) 42
  [arXiv:1207.7152 [hep-ph]].


%%%%% supersoft op as WZW

\bibitem{Alves:2015kia}
  D.~S.~M.~Alves, J.~Galloway, M.~McCullough and N.~Weiner,
  %``Goldstone Gauginos,''
  Phys.\ Rev.\ Lett.\  {\bf 115} (2015) 16,  161801
  [arXiv:1502.03819 [hep-ph]].

% 1:1.5:2.4
\bibitem{Alves:2015bba}
  D.~S.~M.~Alves, J.~Galloway, N.~Weiner and M.~McCullough,
  %``Models of Goldstone Gauginos,''
  arXiv:1502.05055 [hep-ph].

%%%%% Adjoint mass problem

\bibitem{Carpenter:2010as}
  L.~M.~Carpenter,
  %``Dirac Gauginos, Negative Supertraces and Gauge Mediation,''
  JHEP {\bf 1209} (2012) 102
  [arXiv:1007.0017 [hep-th]].

\bibitem{Csaki:2013fla}
  C.~Csaki, J.~Goodman, R.~Pavesi and Y.~Shirman,
  %``The $m_D-b_M$ problem of Dirac gauginos and its solutions,''
  Phys.\ Rev.\ D {\bf 89} (2014) 5,  055005
  [arXiv:1310.4504 [hep-ph]].


\bibitem{Arvanitaki:2013yja}
  A.~Arvanitaki, M.~Baryakhtar, X.~Huang, K.~van Tilburg and G.~Villadoro,
  %``The Last Vestiges of Naturalness,''
  JHEP {\bf 1403} (2014) 022
  [arXiv:1309.3568 [hep-ph]].

%%%%% D-suppression as a prediction

\bibitem{Unwin:2012fj}
  J.~Unwin,
  %``R-symmetric High Scale Supersymmetry,''
  Phys.\ Rev.\ D {\bf 86} (2012) 095002
  [arXiv:1210.4936 [hep-ph]].

\bibitem{Fox:2014moa}
  P.~J.~Fox, G.~D.~Kribs and A.~Martin,
  %``Split Dirac Supersymmetry: 
  %An Ultraviolet Completion of Higgsino Dark Matter,''
  Phys.\ Rev.\ D {\bf 90} (2014) 7,  075006
  [arXiv:1405.3692 [hep-ph]].


%%%%% R mediation

\bibitem{Blechman:2009if}
  A.~E.~Blechman,
  %``R-symmetric Gauge Mediation and the Minimal R-Symmetric
  %Supersymmetric Standard Model,''
  Mod.\ Phys.\ Lett.\ A {\bf 24} (2009) 633
  [arXiv:0903.2822 [hep-ph]].


\bibitem{Kribs:2010md}
 G.~D.~Kribs, T.~Okui and T.~S.~Roy,
  %``Viable Gravity-Mediated Supersymmetry Breaking,''
  Phys.\ Rev.\ D {\bf 82} (2010) 115010
%  doi:10.1103/PhysRevD.82.115010
  [arXiv:1008.1798 [hep-ph]].

%%%%% pmoduli

\bibitem{Intriligator:2007cp}
  K.~A.~Intriligator and N.~Seiberg,
  %``Lectures on Supersymmetry Breaking,''
  Class.\ Quant.\ Grav.\  {\bf 24} (2007) S741
  [hep-ph/0702069].


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% unification and higgs mass


%%%%% fat Higgs

\bibitem{Harnik:2003rs}
  R.~Harnik, G.~D.~Kribs, D.~T.~Larson and H.~Murayama,
  %``The Minimal supersymmetric fat Higgs model,''
  Phys.\ Rev.\ D {\bf 70} (2004) 015002
%  doi:10.1103/PhysRevD.70.015002
  [hep-ph/0311349].


%SU(3)^3
%\bibitem{Rizov:1981dp}
%  V.~A.~Rizov,
%  %``A Gauge Model of the Electroweak and Strong Interactions 
%  %Based on the Group SU(3)$_L$ X SU(3)$_R$ X SU(3)$_c$,''
%  Bulg.\ J.\ Phys.\  {\bf 8} (1981) 461.

\bibitem{trinification1}
  Y.~Achiman and B.~Stech, 
  ``New Phenomena in Lepton-Hadron Physics'', 
  D.E.C.~Fries and J.~Wess eds., Plenum, New York, U.S.A. (1979),
  pg.~303.
\bibitem{trinification2}
  A.~de~Rujula, H.~Georgi and S.L.~Glashow, 
  ``Fifth Workshop on Grand Unification'', 
  K.~Kang, H.~Fried and P.~Frampton eds., 
  World Scientific, Singapore (1984), pg.~88.

%%%%% model with light chiral adjoint

\bibitem{Kakizaki:2013eba}
  M.~Kakizaki, S.~Kanemura, H.~Taniguchi and T.~Yamashita,
  %``Higgs sector as a probe of supersymmetric grand unification 
  %with the Hosotani mechanism,''
  Phys.\ Rev.\ D {\bf 89} (2014) 7,  075013
  [arXiv:1312.7575 [hep-ph]].

\bibitem{Nojiri:2007jm}
  M.~M.~Nojiri and M.~Takeuchi,
  ``The Study of ~q(L) ~q(L) production at CERN LHC 
  in the l+- l+- channel and sensitivity to other models,''
  Phys.\ Rev.\ D {\bf 76} (2007) 015009
  [hep-ph/0701190].


%%%%% 2-loop calculation for higgs mass (improved ver. of SARAH)

%%% for NMSSM:
%\bibitem{Goodsell:2014pla}
%  M.~D.~Goodsell, K.~Nickel and F.~Staub,
%  %``Two-loop corrections to the Higgs masses in the NMSSM,''
%  Phys.\ Rev.\ D {\bf 91} (2015) 035021
%%  doi:10.1103/PhysRevD.91.035021
%  [arXiv:1411.4665 [hep-ph]].

%%%% for MRSSM:
%\bibitem{Diessner:2015yna}
%  P.~Diessner, J.~Kalinowski, W.~Kotlarski and D.~Stockinger,
%  %``Two-loop correction to the Higgs boson mass in the MRSSM,''
%  Adv.\ High Energy Phys.\  {\bf 2015} (2015) 760729
%%  doi:10.1155/2015/760729
%  [arXiv:1504.05386 [hep-ph]].


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% invisible decay 

%%%%% invisible Higgs decay
\bibitem{Belanger:2013kya}
  G.~Belanger, B.~Dumont, U.~Ellwanger, J.~F.~Gunion and S.~Kraml,
  %``Status of invisible Higgs decays,''
  Phys.\ Lett.\ B {\bf 723} (2013) 340
  [arXiv:1302.5694 [hep-ph]].

%%%%% PDG
\bibitem{Agashe:2014kda}
  K.~A.~Olive {\it et al.} [Particle Data Group Collaboration],
  %``Review of Particle Physics,''
  Chin.\ Phys.\ C {\bf 38} (2014) 090001.

\bibitem{Okawa:2013hda}
  H.~Okawa, J.~Kunkle and E.~Lipeles,
  %``Prospects on the search for invisible Higgs decays 
  %in the ZH channel at the LHC and HL-LHC: A Snowmass White Paper,''
  arXiv:1309.7925 [hep-ex].

\bibitem{Asner:2013psa}
  D.~M.~Asner {\it et al.},
  %``ILC Higgs White Paper,''
  arXiv:1310.0763 [hep-ph].

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% appendix
%%%%% SARAH for RGEs 

\bibitem{Staub:2008uz}
  F.~Staub,
  %``Sarah,''
  arXiv:0806.0538 [hep-ph].

\bibitem{Staub:2012pb}
  F.~Staub,
  %``SARAH 3.2: Dirac Gauginos, UFO output, and more,''
  Comput.\ Phys.\ Commun.\  {\bf 184} (2013) 1792
  [arXiv:1207.0906 [hep-ph]].

\bibitem{Staub:2013tta}
  F.~Staub,
  %``SARAH 4 : A tool for (not only SUSY) model builders,''
  Comput.\ Phys.\ Commun.\  {\bf 185} (2014) 1773
  [arXiv:1309.7223 [hep-ph]].


%%%%% RGE

%\bibitem{Degrassi:2012ry}
%  G.~Degrassi, S.~Di Vita, J.~Elias-Miro, J.~R.~Espinosa,
%  G.~F.~Giudice, G.~Isidori and A.~Strumia,
%  %``Higgs mass and vacuum stability in the Standard Model at NNLO,''
%  JHEP {\bf 1208} (2012) 098
%  [arXiv:1205.6497 [hep-ph]].

\bibitem{Buttazzo:2013uya}
  D.~Buttazzo, G.~Degrassi, P.~P.~Giardino, G.~F.~Giudice, 
  F.~Sala, A.~Salvio and A.~Strumia,
  %``Investigating the near-criticality of the Higgs boson,''
  JHEP {\bf 1312} (2013) 089
  [arXiv:1307.3536 [hep-ph]].

%\bibitem{Bezrukov:2012sa}
%  F.~Bezrukov, M.~Y.~Kalmykov, B.~A.~Kniehl and M.~Shaposhnikov,
%  %``Higgs Boson Mass and New Physics,''
%  JHEP {\bf 1210} (2012) 140
%  [arXiv:1205.2893 [hep-ph]].


%\bibitem{Machacek:1983tz}
%  M.~E.~Machacek and M.~T.~Vaughn,
%  %``Two Loop Renormalization Group Equations in a General Quantum
%  %Field Theory. 1. Wave Function Renormalization,''
%  Nucl.\ Phys.\ B {\bf 222} (1983) 83;
%%
%%\bibitem{Machacek:1983fi}
%%  M.~E.~Machacek and M.~T.~Vaughn,
%  %``Two Loop Renormalization Group Equations in a General Quantum
%  %Field Theory. 2. Yukawa Couplings,''
%%  Nucl.\ Phys.
%	\textit{ibid} \ B {\bf 236} (1984) 221;
%%
%%\bibitem{Machacek:1984zw}
%%  M.~E.~Machacek and M.~T.~Vaughn,
%  %``Two Loop Renormalization Group Equations in a General Quantum
%  %Field Theory. 3. Scalar Quartic Couplings,''
%%  Nucl.\ Phys.
%	\textit{ibid}	\ B {\bf 249} (1985) 70.

\bibitem{Luo:2002ey}
  M.~x.~Luo and Y.~Xiao,
  %``Two loop renormalization group equations in the standard model,''
  Phys.\ Rev.\ Lett.\  {\bf 90} (2003) 011601
  [hep-ph/0207271].






%\bibitem{Martin:1997ns}
%  S.~P.~Martin,
%  %``A Supersymmetry primer,''
%  Adv.\ Ser.\ Direct.\ High Energy Phys.\  {\bf 21} (2010) 1
%   [Adv.\ Ser.\ Direct.\ High Energy Phys.\  {\bf 18} (1998) 1]
%  [hep-ph/9709356].


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% no used ################


%(NMSSM new)%
%\bibitem{Hagimoto:2015tua}
%  K.~Hagimoto, T.~Kobayashi, H.~Makino, K.~i.~Okumura and T.~Shimomura,
%  %``Phenomenology of NMSSM in TeV scale mirage mediation,''
%  arXiv:1509.05327 [hep-ph].


%no dirac gaugino 

%\bibitem{Abe:2007kf}
%  H.~Abe, T.~Kobayashi and Y.~Omura,
%  %``Relaxed fine-tuning in models with non-universal gaugino masses,''
%  Phys.\ Rev.\ D {\bf 76} (2007) 015002
%  [hep-ph/0703044].
 
%\bibitem{Choi:2006bh}
%  K.~Choi and K.~S.~Jeong,
%  %``Supersymmetry breaking and moduli stabilization with anomalous
%  %U(1) gauge symmetry,''
%  JHEP {\bf 0608} (2006) 007
%  [hep-th/0605108].

%\bibitem{Goodsell:2015ura}
%  M.~D.~Goodsell, M.~E.~Krauss, T.~Mueller, W.~Porod and F.~Staub,
%  %``Dark matter scenarios in a constrained model with Dirac gauginos,''
%  JHEP {\bf 1510} (2015) 132
%  [arXiv:1507.01010 [hep-ph]].




%\bibitem{Ding:2015epa}
%  R.~Ding, T.~Li, F.~Staub and B.~Zhu,
%  %``The Supersoft and Super-Natural Supersymmetry,''
%  arXiv:1510.01328 [hep-ph].


%\bibitem{Bhattacharyya:2012qj}
%  G.~Bhattacharyya and T.~S.~Ray,
%  %``Pushing the SUSY Higgs mass towards 125 GeV with a color adjoint,''
%  Phys.\ Rev.\ D {\bf 87} (2013) 1,  015017
%  [arXiv:1210.0594 [hep-ph]].


%\bibitem{Bertuzzo:2014sma}
%  E.~Bertuzzo and C.~Frugiuele,
%  %``A natural SM-like 126 GeV Higgs via non-decoupling D-terms,''
%  arXiv:1412.2765 [hep-ph].


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%	
\end{thebibliography}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\end{document}

